Mind the Gap? Not for SVP Hardness under ETH!

We prove new hardness results for fundamental lattice problems under the Exponential Time Hypothesis (ETH). Building on a recent breakthrough by Bitansky et al.\ \cite{BHIRW24}, who gave a polynomial-time reduction from $\mathsf{3SAT}$ to the (gap) $\mathsf{MAXLIN}$ problem-a class of CSPs with linear equations over finite fields-we derive ETH hardness for several lattice problems. First, we show that for any $p \in [1, \infty)$, there exists an explicit constant $\gamma > 1$ such that $\mathsf{CVP}_{p,\gamma}$ (the $\ell_p$-norm approximate Closest Vector Problem) does not admit a $2^{o(n)}$-time algorithm unless ETH is false. Our reduction is deterministic and proceeds via a direct reduction from (gap) $\mathsf{MAXLIN}$ to $\mathsf{CVP}_{p,\gamma}$. Our main contribution is a randomized ETH hardness result for $\mathsf{SVP}_{p,\gamma}$ (the $\ell_p$-norm approximate Shortest Vector Problem) for all $p \in (2, \infty)$. This result relies on a novel geometric property of the integer lattice $\mathbb{Z}^n$ in the $\ell_p$ norm, which says that for any $p \in (2, \infty)$, the number of lattice vectors close to $\frac{1}{2}\vec{1}_n$ (in the $\ell_p$ norm) is exponentially larger than the number of short vectors (namely those close to the origin). We establish this property via a new inequality for the Theta function, which we use to get a randomized reduction from $\mathsf{CVP}_{p,\gamma}$ to $\mathsf{SVP}_{p,\gamma'}$. Finally, we also use our ideas to give some minor improvements over prior reductions from $\mathsf{3SAT}$ to $\mathsf{BDD}_{p,\alpha}$ (the Bounded Distance Decoding Problem), yielding better ETH hardness results for $\mathsf{BDD}_{p,\alpha}$ for any $p \in [1, \infty)$ and $\alpha > \alpha_p^{\ddagger}$, where $\alpha_p^{\ddagger}$ is an explicit threshold depending on $p$.

==> 4_svp.tex <==


In this section we show a reduction from $\sat$ in $n$ variables to $\svp_{p, \gamma}$ in a lattice of rank $\order{n}$. We do this by proving a reduction from $\cvp_{p, \gamma'}$ for a constant $\gamma'$ (as obtained in \cref{sec:cvp_hard}) to $\svp_{p, \gamma}$ for a constant $\gamma$. The result then follows from combining the reduction from $\sat$ to $\lin$ in \cref{thm:satToLinRed}, and from $\lin$ to $\cvp$ in \cref{thm:LinCvpReduction}. We first show that a family of lattice gadget-target pairs exist, which will be used in the reduction.

\subsection{Locally Dense Integer Lattices}
\label{ssec:locally_dense_lattices}

We wish to show that in the integer lattice $\Z^n$, there are exponentially more vectors close to $\frac{1}{2}\vec 1_n$ than the number of {\em short} vectors. The following property of the theta function will be useful. 

\begin{lemma}
    \label{lem:thetaProp}
    For every $p \geq 2+10^{-7}$, there exists a $\tau > 0$ such that 
    \begin{equation}
        \label{eqn:thetaProp}
        \Theta_p(\tau, 0) < \Theta_p(\tau, 1/2). 
    \end{equation}
    % Furthermore, $\tau$ can be efficiently computed from $p$.
\end{lemma}

\begin{proof}
% \adi{To be revised thoroughly.}

From the definition, 
\[\Theta_p(\tau,0) = \sum_{z \in \Z} e^{-\tau|z|^p} = 1+ 2 \sum_{z =1}^{\infty} e^{-\tau\cdot z^p},\]
and 
\[\Theta_p(\tau,1/2) = \sum_{z \in \Z} e^{-\tau|z-1/2|^p} =  2 \sum_{z =1}^{\infty} e^{-\tau \cdot (z-1/2)^p}.\]
      %%%%%%%%%%%%%%%%%%%
      %%%%%%%%%%%%%%%%%%%
Define 
\[ A_z(p, \tau) := e^{-\tau (z - 1/2)^p} - e^{-\tau z^p}, \]
% \[ \Delta(p,\tau) := \sum_{z = 1}^{\infty} A_z(p, \tau) = \sum_{z = 1}^{\infty} \paren{ e^{-\tau (z - 1/2)^p} - e^{-\tau z^p} }. \]
% and
\[
S_n(p,\tau) := \sum_{z=1}^{n} A_z(p,\tau)
\]
The condition $\Theta_p(\tau,0)<\Theta_p(\tau,1/2)$ is equivalent to,\[S_\infty(p,\tau)>0.5\]
Observe that $\forall z \geq 1,~A_z > 0$. It is enough to show that for $p \geq 2.001$, there exists $n \in \N, \tau>0$ such that $S_n(p,\tau) > 1/2.$ 
Also,
\[ \frac{\partial A_z(p, \tau)}{\partial p} = -\tau\cdot \left( e^{-\tau \cdot (z-0.5)^p} (z-0.5)^p \ln(z-0.5) - e^{-\tau\cdot z^p} z^p \ln z \right) \]


      
\textbf{Suppose $p\geq 2.2$.} We claim that in this case, $\exists \tau > 0$ such that $\forall p \geq 2.2,~S_1(p, \tau) = A_1(p, \tau) > 1/2.$ Differentiating $A_1(p, \tau)$ with respect to $p$, we see that
\[
\frac{\partial A_1(p, \tau)}{\partial p} = \tau e^{-\tau (1/2)^p} \cdot (1/2)^p \cdot \ln(2) >0.
\]
This implies that $A_1(p, \tau)$ is increasing with respect to $p$. Therefore it suffices to find a $\tau>0$ such that $A_1(\tau,2.2)>0.5$. 
Conveniently, we find that for $\tau = 1.949$, $~A_1(2.2, 1.949) > 0.5$\footnote{This $\tau$ is chosen such that it is close to the maximizer of $A_1(\tau, 2.2).$}. 
% \tau=\frac{2^{2.2}\ \ln(2^{2.2})}{2^{2.2}-1}

\textbf{Suppose $p \in [2.001, 2.2)$.}\footnote{From here on, since the proof is somewhat computational, the reader may use the following script to verify the work on \href{https://colab.research.google.com/drive/1T-4dKo1LHMgMow1UGGgBRdY-2aslCjq1?usp=sharing}{Colab}. Additionally, a \href{https://www.desmos.com/calculator/i3tzezgkzq}{Desmos} link with a plot of the feasible region is available.} 
We will truncate the series $S_{\infty}$ to the first ten terms and fix $\tau = \tau_0 := 0.89$. Define
\[h(p) = S_{10}(p,0.89) = \sum_{z=1}^{10} e^{- \tau_0 \cdot (z-0.5)^p}- e^{-\tau_0 \cdot z^p}.\]
We claim that for $2.001 \leq p <2.2$, $h(p)>0.5$. To see that, consider the derivatives with respect to $p$,
\[
h'(p) = \sum_{z=1}^{10} -\tau_0\cdot \left( e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p \ln(z-0.5) - e^{-\tau_0\cdot z^p} z^p \ln z \right)
\;,\]
and, 
\begin{align}
h''(p) = \tau_0^2\cdot\sum_{z=1}^{10}  \left( e^{- \tau_0 \cdot(z-0.5)^p} (z-0.5)^{2p} (\ln(z-0.5))^2 \right)+\tau_0\sum_{z= 1}^{10}\left( e^{-\tau_0\cdot z^p} z^p (\ln z )^2\right) \notag \\
-\tau_0^2\sum_{z=1}^{10}\left( e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 \right) -\tau_0\cdot \sum_{z=1}^{10} \left( e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2\right).
\label{eqn:uglyproof1}
\end{align}
We wish to find an $L>0$ such that if $2.001\leq p < 2.2$, then $-L\leq h''(p)$. For that, we collect all the negative terms from \cref{eqn:uglyproof1} and get the following bound,
\[h''(p)>-\tau_0^2 \left(\sum_{z=2}^{10} e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 \right)-\tau_0\left( \sum_{z=2}^{10} e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2\right) -\frac{\tau_0 e^{-\tau_0/2^p} \cdot (\ln{2})^2}{2^p}.\] 
Since $2<p\leq 2.2$, using the fact that for $x>1$ and 
\begin{align}
    e^{-\tau_0 \cdot x^p}<e^{-\tau_0 \cdot x^2} \text{ and } x^{2p}<x^{5} \label{eqn:weirdineq1} ,\\
     e^{-\tau_0 \cdot x^p}<e^{-\tau_0 \cdot x^2} \text{ and } x^{p}<x^{3} \label{eqn:weirdineq2}.
\end{align}
we get that for $z\geq2$,
\begin{align*}
   % z^{2p}<z^5,e^{-\tau_0 \cdot z^p}\leq e^{-\tau_0\cdot z^2}\implies 
   e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 &\leq e^{-\tau_0 \cdot z^2} z^{5}(\ln z)^2; && \text{(from \cref{eqn:weirdineq1})}\\
    % (z-0.5)^{p}<(z-0.5)^3,e^{-\tau_0 \cdot (z-0.5)^p}\leq e^{-\tau_0\cdot (z-0.5)^2}\implies
    e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2 & \leq e^{-\tau_0 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2; && \text{(from \cref{eqn:weirdineq2})}\\
    \frac{e^{-\tau_0 / 2^p}  (\ln 2)^2}{2^p} &\leq \frac{e^{-\tau_0/8} \cdot (\ln{2})^2}{4}.
\end{align*}
This implies that for all $2.001\leq p \leq 2.2$,
\begin{align*}
h''(p)&>\:-\tau_0^2 \left(\sum_{z=2}^{10}  e^{-\tau_0 \cdot z^2} z^{5} (\ln z)^2 \right) -\tau_0\left( \sum_{z=2}^{10} e^{-\tau_0 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2\right) -\frac{\tau_0 e^{-\tau_0/8} \cdot (\ln{2})^2}{4} \\ & >\;(-0.64).
\end{align*}
%%%%%%


%%%%%%
Notice that for any finite $z \in \Z$, $A_z(p, \tau)$ is a smooth function. Therefore a finite truncation of the sum $S_{\infty}$ is a smooth function. Hence, we can use Taylor's theorem \cite[Theorem 6.4.1]{bartle} to bound the values in the intervals $2.001 \leq p \leq 2.1 $ and $2.1 \leq p \leq 2.2$. 
Let $\Delta = (p-2.001)$. By Taylor's theorem, for any $p \in[2.001,2.1]$, there exists a $p'\in[2.001, p]$ such that,  
$$h(p) = h(2.001)+ h'(2.001)\cdot \Delta+\frac{h''(p')\cdot\Delta^2}{2} \:.$$ 
We have that $h(2.001)\geq 0.50000971 >0.5$ and $h'(2.001)\geq 0.067056759$. Since $h'(2.001)>0$, and $\Delta \in [0,0.099]$ then
using the fact that $h''(p')>-0.64$ we get that,
$$h(p)\geq\min_{\Delta \in[0,0.099]}\left\{h(2.001)+h'(2.001)\cdot\Delta-\frac{ (0.64)\Delta^2}{2} \right\} \:.$$
Let, $$q(\Delta)= h(2.001)+h'(2.001)\cdot\Delta-\frac{(0.64) \Delta^2}{2} \:.$$
Since $q $ is an inverted parabola, the minimum on the interval $[0,0.099]$ must be attained at one of the end points of the interval and we get that $q(0)=h(2.001)>0.5$ and $q(0.099)\geq  0.5035>0.5$.
Similarly since $h(2.1)\geq 0.50623643$ and $h'(2.1)\geq 0.05875258>0$ for all $p\in[2.1,2.2]$ we get that,
\begin{align*}
h(p)&\geq \min_{\Delta \in[0,0.1]}\left\{h(2.1)+h'(2.1)\cdot\Delta-\frac{ (0.64)\Delta^2}{2} \right\} \: .\end{align*}
Now again let, 
$$q_1(\Delta)= h(2.1)+h'(2.1)\cdot\Delta-\frac{(0.64) \Delta^2}{2} \:.$$
Again, since $q_1$ is an inverted parabola, we get that for all $p\in[2.1,2.2]$, $h(p)\geq \min \left\{q_1(0), q_1(0.1)\right\}$. Since $q_1(0)=h(2.1)>0.5$ and $q_1(0.1)\geq 0.5089>0.5$, we get that $h(p)>0.5$ for all $p \in [2.001,2.2]$.

\textbf{Suppose} $p \in [2+10^{-7}, 2.001)$. Take $\tau_1=0.162665$ and $h(p) = S_{11}(p, \tau_1)$.
Using an argument along similar lines as that in the previous case, we get that for all $2+10^{-7}\leq p \leq 2.001$,
\begin{align*}
h''(p)&>\:-\tau_1^2 \left(\sum_{z=2}^{11}  e^{-\tau_1 \cdot z^2} z^{5} (\ln z)^2 \right) -\tau_1\left( \sum_{z=2}^{11} e^{-\tau_1 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2\right) -\frac{\tau_1 e^{-\tau_1/8} \cdot (\ln{2})^2}{4} \\ & >\;(-16.5).
\end{align*}

This time, we have that $h(2+10^{-7})\geq 0.50000000051525>0.5$ and $h'(2+10^{-7})\geq0.009104222964$. Therefore, by Taylor's Theorem we get that for all $p\in [2+10^{-7},2.001]$,
\begin{align*}
    h(p) &\geq  \min_{\Delta \in[0,0.001]}\left\{h(2+10^{-7})+h'(2+10^{-7})\cdot\Delta-\frac{ (16.5)\Delta^2}{2} \right\}\\
    &\geq \min\left\{h(2+10^{-7}), 0.5000008\right\}\\
    &>0.5
\end{align*}
\end{proof}


\begin{theorem}
    \label{thm:SvpIntegerGadget}
    For any $p \geq 2+10^{-7},~\sigma > 1$, there exists constants $\delta \in (0, 1/2)$, $\phi_0, \phi_1 > 1$ and $C_r>0$, such that for any $n \in \Z^+$, if $r :=C_r \cdot {n^{1/p}}$ then the following holds for the integer lattice. 
    \begin{align}
        \nump{\Z^{n}, (1-\delta)^{1/p} r, \frac{1}{2}\vec{1}_{n}} \geq \max\bigg\{ &\phi_0^{n - o(n)} \nump{\Z^{n}, r, \vec{0}}, \notag \\
        &\phi_1^{n - o(n)} \nump{\Z^{n}, (1-\delta\sqrt{\sigma})^{1/p} r, \frac{1}{2} \vec{1}_{n}} \bigg\}.
        \label{eqn:SvpIntegerGadgetCond}
    \end{align} 
     The constants $\delta, \phi_0, \phi_1, C_r$ only depend  upon $p$ and can be efficiently computed with required precision, from $p$. 
\end{theorem}

% \adi{To be revised thoroughly.}   
% \adi{Change $\dgr m$ to $n$, $\dgr r$ to $r$.}
% \adi{Use appropriate macros and restatables instead of rewriting.}
% \adi{Equation spacing is fucked up.}
% \adi{Write that the constants can be estimated efficiently, reformulate that theorem properly and check the quatification.}

\begin{proof}
Fix any $p$ and $\sigma$. Fix $\tau > 0$ as in \cref{lem:thetaProp}. Then define 
$$\rho:=\frac{\Theta_p(\tau,1/2)}{\Theta_p(\tau,0)}>1.$$ 
Notice that the precision to which we would approximate $\rho$ would be independent of the input size, so such a $\rho$ is efficiently computable in constant time. 
For a $\delta \in (0, 1/2)$ to be determined in what follows, fix 
$$C_r := \frac{\mu_p(\tau,1/2)^{1/p}}{(1-\delta)^{1/p}}.$$
 By \cref{thm:theta_gives_good_approx}, there exists a constant $C^*>0$ such that,

\begin{equation}
\label{eq:bd1}
\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}} \geq \exp\left(-C^* \sqrt{n}\right)\cdot \exp(\tau n \cdot \mu_p(\tau,1/2))\cdot \Theta_p(\tau , 1/2)^{n}.
\end{equation}

By \cref{lemma:theta0}, 
\begin{equation}
\label{eq:bd2}
\nump{\Z^{n},r,\vec{0}} \leq \exp\paren{\tau \cdot\frac{n ~\mu_p(\tau,1/2)}{1-\delta}}\cdot \Theta_p(\tau,0)^{n}.
\end{equation}
% \[N_p(2\Z^{m^\dagger},r^\dagger,0)\leq \exp\paren{\tau \cdot\frac{m^\dagger \cdot \mu_p(\tau,1/2)}{1-\delta}}\cdot \Theta_p(\tau,0)^{m^\dagger}\]
From \cref{eq:bd1,eq:bd2}, we get that 
\[\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}}}{\nump{\Z^{n},r,\vec{0}}} \geq \rho^{n} \cdot \exp\left(-C_r^p\tau\delta n -o(n)\right).\]
Because $\rho>1$, we can fix $\delta>0$ such that,
$$\delta < \frac{\log \rho}{\tau \mu_p(\tau, 1/2) + \log \rho},$$
which implies that $\rho \cdot \exp(-\tau \delta C_r^p)>1$. 
Then set $\phi_0:=\rho \cdot \exp(-\tau \delta C_r^p)$. This implies that, 
$$\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}}}{\nump{\Z^{n},r, \vec{0}}} \geq \phi_0^{n -o(n)}.$$

For the second inequality, again use \cref{lemma:theta0} to get,
\begin{equation}
\label{eq:bd3}
N_p\left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}\right)\leq \Theta_p(\tau,1/2)^{n} \cdot \exp\paren{\tau \cdot n C_r^p \cdot (1-\delta\sqrt{\sigma})}.
\end{equation}
Then set  $\phi_1:=\exp \paren{\tau\delta C_r^p\cdot(\sqrt{\sigma}-1)}>1$ which implies,
\[\frac{N_p\left(\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}\right)}{N_p \left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n} \right)}\geq \exp \paren{\tau\delta n C_r^p\cdot(\sqrt{\sigma}-1) -o(n)}=\phi_1^{n-o(n)}. \]
\end{proof}




We conjecture the following.
\begin{conjecture}
\label{conj:the_conjecture}
    For every $p>2$ there exists a $\tau>0$, such that,
    \[\Theta_p(\tau,1/2)>\Theta_p(\tau,0)\]
\end{conjecture}
If the above conjecture is proved to be true it will imply \cref{thm:linToSvp} for every $p>2$.
\subsection{From \texorpdfstring{$\lin_\varepsilon$}{MAXLIN varepsilon} to \texorpdfstring{$\svp_{p, \gamma}$}{SVP p, gamma}}

In the following, we  start with a $\cvp_{p, \gamma'}$ instance with the special property that twice the target vector is in the lattice, and find a lattice $\cL$ and a parameter $r$ such that the number of vectors in $\cL$ of length at most $r$ are $2^{\Omega(n)}$ times more for a YES instance than for a NO instance. 
\begin{lemma}
    \label{lem:cvpToSvp}
    Suppose $(B', \vec t', r')$ is a $\cvp_{p, \gamma'}$ instance over an integer lattice %\dnote{The CVP instance type should match the definition, i.e., instead of being given a lattice, you should be given a generating set. Then the rank $n$ should be replaced by the number of columns in the generating set.}
    such that $B \in \Z^{m \times m'}, \vec t' \in \lat(B') / 2$ and $\vec t' \in \Z^m$. Then for any $d \in \Z^+, \alpha > 0$ there exists an efficiently computable matrix $B$ that generates a lattice $\lat(B)$ in $m + d + 1$ dimensions such that for any constants $\gamma'$ and any radii $r_G$,$r_A$,
    \begin{enumerate}
        \item If $\di_p\paren{\vec{t}',\cL(B')}\leq r'$  then,
        \begin{equation}
            \label{eqn:cvpToSvpYes}
        \nump{\lat, r_G, \vec 0} \geq \nump{\alpha \Z^{d}, (r_G^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}},
    \end{equation}
        \item If  $\di_p\paren{\vec{t}',\cL(B')}> \gamma'r'$ then,
        \begin{align}
            \label{eqn:cvpToSvpNo}
        \nump{\lat, r_A, \vec 0} \leq \paren{\floor{r_A} + 1} \nump{\Z^n, r_A, \vec 0} \bigg( &\nump{\alpha \Z^{d}, (r_A^p - (\gamma' r')^p)^{1/p}, \frac{\alpha}{2}\vec{1}_d} \notag \\ &+ \nump{\alpha \Z^{d}, r_A, \vec 0} \bigg).
    \end{align}
    \end{enumerate}
\end{lemma}

\begin{proof}
% \dnote{The input is given in terms of the generating set. Also, $B$ will define the generating set of $\cL$.}
    % Let $B'$ be a basis for $\lat'$.
    Fix any valid $d, \alpha$. 
    Define $\dgr B := \alpha I_{d}$, $\vec t^{\dagger} := \frac{\alpha}{2}\vec{1}_{d}$.
    Define
    \begin{equation}
        \label{eqn:cvpToSvpBasis}
    B := \begin{pmatrix}
        B' & 0 & -\vec t' \\
        0 & \dgr{B} & - \vec{t}^{\dagger} \\
        0 & 0 & 1
    \end{pmatrix}. 
    \end{equation}
    Then $\lat = \lat(B)$ is a lattice in $m + d + 1$ dimensions, and $B$ is clearly efficiently computable. 
    Let $\dgr \lat = \lat(\dgr B)$. 
    Suppose that the input $\cvp_{p, \gamma'}$ instance was a \yes instance. This implies that $\dist(\cL', \vec t') \leq r'$. Then $\exists \vec x \in \Z^{m'}$ such that $\norm{B'\vec x - \vec t'}_p \leq r'$. 
    For any $r_G$, consider a vector $\vec v \in \ballp{\ldgr, (r_G^p - 1 - r'^p)^{1/p}, \tdgr}$ such that $\vec v = \dgr B \vec y$ for some $\vec y \in \Z^{d}$. Then the vector $\vec u := B \cdot (\vec x, \vec y, 1)$ satisfies
    $$ \normpp{\vec u} \leq \normpp{B'\vec x - \vec t} + \normpp{\dgr B \vec y - \tdgr} + 1 \leq r_G^p. $$
    Therefore, $\vec u \in \ballp{\lat, r_G, \vec 0}$. Since this mapping between $\vec v$ and $\vec u$ is injective, we have that
    $$ \nump{\lat, r_G, \vec 0} \geq \nump{\dgr B, (r_G^{p} - 1 - r'^p)^{1/p}, \tdgr}. $$
    This completes the proof of item 1. 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Next, suppose that the input $\cvp_{p, \gamma'}$ instance was a \no instance. This implies that $\dist(\cL', \vec t') > \gamma' r'$. 
    For any $r_A$, let $\vec u \in \ballp{\lat, r_A, \vec 0}$ such that $\vec u = (B'\vec x, B^\dagger \vec y , \cl)$ for some $\vec x \in \Z^{m'},~\vec y\in\Z^d$ and $\cl\in \Z$. We have 
    \[ \normpp{\vec u} \leq \normpp{B'\vec x - \cl\vec t'} + \normpp{\dgr B \vec y - \cl\tdgr} + \cl^p \leq r_A^p, \]
    which implies that 
    \[ \normpp{B'\vec x - \cl \vec t'} \leq r_A^p - \cl^p \leq r_A^p; \]
    \begin{equation}
    \label{eqn:coeffForGadget}
     \normpp{\dgr B \vec y - \cl \vec t^{\dagger}} ~\leq ~r_A^p - \cl^p - (\dist_p(\lat', \ell \vec t'))^p ~\leq ~r_A^p - (\dist_p(\lat', l \vec t'))^p.
     \end{equation}
    Since $\lat' \subseteq \Z^m$, and $\cl \vec t' \in \Z^m$, we have that the number of values that $B'\vec x$ can take is 
    \begin{align}
        \nump{\lat', r_A, \cl \vec t'} \notag &\leq \nump{\Z^m, r_A, \cl \vec t'} && (\because \lat \subseteq \Z^m) \notag \\
        &= \nump{\Z^m, r_A, \vec 0} && (\because \cl\vec t' \in \Z^m) \label{eqn:svptemp1}.
    \end{align}
    
    Let $S_\cl$ be the set of points in $\lat$ of length at most $r_A$ such that their last coordinate is $\cl$. Observe that $\abs{S_\cl} = \abs{S_{-\cl}}$. 
    Then, 
    $$ \nump{\lat, r_A, \vec 0} \leq \sum_{\cl=-\floor{r_A}}^{\floor{r_A}} \abs{S_\cl} \leq 2 \sum_{\cl = 0}^{\floor{r_A}} \abs{S_\cl}. $$

    \textbf{Suppose that $\cl$ is even.} Then $\vec t' \in \lat' / 2 \implies \dist_p(\lat', \cl\vec t') = 0$ and $\cl \tdgr \in \ldgr$. Thus, we have that the number of possible values $\vec B^\dagger y$ can take is at most,
    \begin{align}
        \label{eqn:svptemp2}
        \nump{\ldgr, r_A, \cl \tdgr} = \nump{\ldgr, r_A, \vec 0}.
    \end{align}
    The number of possible vectors $\vec u$ in this case is at most the product of \cref{eqn:svptemp1} and \cref{eqn:svptemp2},
    \begin{align}
        \label{eqn:svpslodd}
        \abs{S_l} \leq \nump{\Z^m, r_A, \vec 0} \nump{\ldgr, r_A, \vec 0}.
    \end{align}
    \textbf{Suppose that $\cl$ is odd.} Then $\vec t' \in \lat' / 2 \implies \cl\vec t' \in \lat' + \vec t'$. Let $\cl = 2z+1$. We have that
    $$\dist_p(\lat', (2z+1)\vec t') = \dist_p(\lat', \vec v' + \vec t') = \dist_p(\lat', \vec t'),$$
    where $\vec v' \in \lat'$. 
    Therefore, the number of possible values $B^\dagger \vec y$ can take while satisfying \cref{eqn:coeffForGadget} is at most 
    % \rnote{Can you elaborate more on this step}
    \begin{align}
        \label{eqn:svptemp3}
        % \nump{\ldgr, (r_A^p - \cl^p - (\gamma' r')^p)^{1/p}, \cl \tdgr} \leq 
        \nump{\ldgr, (r_A^p - (\gamma' r')^p)^{1/p}, \cl \tdgr} 
        = \nump{\ldgr, (r_A^p - (\gamma' r')^p)^{1/p}, \tdgr}.
    \end{align}
    The number of possible vectors $\vec u$ in this case is at most the product of \cref{eqn:svptemp1} and \cref{eqn:svptemp3},
    \begin{align}
        \label{eqn:svpsleven}
        \abs{S_l} \leq \nump{\Z^m, r_A, \vec 0} \nump{\ldgr, (r_A^p - (\gamma' r')^p)^{1/p}, \tdgr}.
    \end{align}
    Thus summing over even and odd $l$ from \cref{eqn:svpslodd} and \cref{eqn:svpsleven},
    \begin{equation}
        \nump{\lat, r_A, \vec 0} \leq (\floor{r_A} + 1) \nump{\Z^m, r_A, \vec 0} \paren{ \nump{\ldgr,~(r_A^p - (\gamma' r')^p)^{1/p},~\tdgr} + \nump{\ldgr, r_A, \vec 0} }.
    \end{equation}
    This completes the proof of item 2.
\end{proof}

% \dnote{We should have a corollary here saying that the number of short vectors in the YES case are exponentially more than the number of short vectors in the NO case. A lot of the calculations, particularly Claim 4.5 in the following theorem will appear in this corollary. Also, don't throw this to the appendix. }

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%

This gives us the following lemma, that says that for any $\lin_\varepsilon$ instance, we can efficiently compute a lattice such that the number of short vectors in the \yes case are exponentially more than the number of short vectors in the \no case. 

\begin{lemma}
    \label{lem:AGRelation}
    For all $p \in [2+10^{-7},\infty)$ , there is an efficient algorithm that takes as an input a $\lin_\varepsilon$ instance $(M, \vec v)$ over $\F_2$ in $n$ variables and $m = \order{n}$ equations, and outputs $(B, r, \gamma, A, G)$ where $B$ generates a lattice $\lat$ in $\order{n}$ dimensions, $\gamma > 1$ is a constant, $r > 0$ is a radius, and constants $A,~G$ are such that $G \geq 2^m A$ and 
    \begin{enumerate}
        \item if it was a \yes instance of $\lin_\varepsilon$ then, $\nump{\lat, r, \vec 0} \geq G$;
        \item if it was a \no instance of $\lin_\varepsilon$ then, $\nump{\lat, \gamma r, \vec 0} \leq A$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    Fix a $p$. We describe the algorithm followed by correctness. 

    \textbf{Algorithm.}
    Define $\gamma' := \paren{1 + \frac{8\varepsilon}{3}}^{1/p}$.
    On input a $\lin_\varepsilon$ instance $M \in \F_2^{m \times n},~\vec v \in \F_2^m$, the reduction computes a $\cvp_{p, \gamma'}$ instance $(B', \vec t', r')$ using the algorithm from \cref{thm:LinCvpReduction}.
    Recall from the proof of \cref{thm:LinCvpReduction} that if this instance is a \yes instance, then $\dist_p(\lat(B'), \vec t') \leq r'$, and if this instance is a \no instance then $\dist_p(\lat(B'), \vec t') \geq (\gamma' r')$. 
    Also recall that by construction in \cref{thm:LinCvpReduction}, $B' \in \Z^{m \times (n+m)}$, $r' = {(3m/8)^{1/p}}$, $2\Z^m \subseteq \lat(B') \subseteq \Z^m$ and $\vec t' \in \lat(B') / 2$ as $\vec t' \in \Z^m$.
    Therefore, this instance satisfies the conditions for \cref{lem:cvpToSvp} to hold. The reduction applies that transformation for a particular choice of efficiently computable parameters $\alpha$, $r$, $\gamma$ and $d$ (to be determined in what follows), to get a generating set $B$ of a lattice $\lat$ in $m + d + 1$ dimensions. 
    Define
    \begin{equation}
        \label{eqn:svpGood}
    G := \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}},
\end{equation}
    \begin{align}
        \label{eqn:svpAnnoying}
        A &:= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \\ 
        &\geq \paren{\floor{\gamma r} + 1} \nump{\Z^m, \gamma r, \vec 0} \paren{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}} + \nump{\alpha \Z^{d}, \gamma r, \vec 0} }. \notag
    \end{align}
    The reduction outputs $(B, \gamma, r, A, G)$. Efficiency is clear, as $A$ and $G$ can be approximated efficiently using the theta function. We will now prove the correctness. 

    \textbf{Correctness.}
    Notice that $G$ and $A$ are simply the RHS of \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo} respectively. \Cref{eqn:svpGood} and \cref{eqn:cvpToSvpYes} imply that if the input was a \yes instance of $\lin_\varepsilon$, then $$\nump{\lat, r, \vec 0} \geq G.$$
    Similarly, \cref{eqn:svpAnnoying} and \cref{eqn:cvpToSvpNo} imply that if the input was a \no instance of $\lin_\varepsilon$, then $$\nump{\lat, \gamma r, \vec 0} \leq A.$$
    Let $\delta$ and $C_r$ be as in \cref{thm:SvpIntegerGadget} for the parameters $(p, \sigma=\gamma'^p)$. Fix $r, \gamma$ such that 
    $$r^p = \svprval; \quad \quad \gamma^p = \svpgammaval.$$
    By \cref{lemma:theta0}, for any $\gamma r,~\tau$, there exists a $K > 0$ such that 

    \begin{align}
        \nump{\Z^{m}, \gamma r, \vec 0} &\leq \exp(\tau (\gamma r)^p) \Theta(\tau, \vec 0) \notag \\ 
        &= \exp(\tau (\gamma r)^p) \Theta(\tau, 0)^{m} \notag \\ 
        &\leq K^{m} && (\because r^p \in \order{m}).
    \label{eqn:numpKsvp}
    \end{align}

    Let $\phi_0, \phi_1$ be the constants from \cref{thm:SvpIntegerGadget} for the particular $p$.
    Set $$d = \max\left\{ \ceil{\log_{\phi_0}(3K)}, \ceil{\log_{\phi_1}(3K)} \right\} m,$$ and let $~\dgr r = C_r \cdot(d)^{1/p}$.
    A simple but tedious calculation shows that the following is true.
    \begin{restatable}{claim}{claimSvpGadgetParam}
        \label{claim:SvpGadgetParameter}
        For any $p,\gamma', r'$, if we set 
        \begin{align*}
        \alpha^p = \svpalphaval;
        \quad \quad r^p = \svprval; 
        \quad \quad \gamma^p = \svpgammaval;
    \end{align*}
    then the following holds. 
    \begin{enumerate}
        \item $\left(r^{p} - 1 - r'^p\right)^{1/p} \geq (1-\delta)^{1/p} (\alpha r^{\dagger})$. \label{im:svpRadii1}
        \item $\gamma r \leq \alpha r^{\dagger}$ \label{im:svpRadii2}
        \item $\left((\gamma r)^p - (\gamma' r')^p \right)^{1/p}\leq (1 - \delta\sqrt{\gamma'^p})^{1/p} (\alpha r^{\dagger})$ \label{im:svpRadii3}
    \end{enumerate}
    \end{restatable}

    To see \cref{im:svpRadii1} notice that,
    \begin{align*}
        r^p-1-r'^p&= \left(1-\frac{\delta}{2} \right)\frac{ 2r'^p}{\delta} - r'^p =2\frac{(1-\delta)}{\delta}r'^p= (1-\delta)(\alpha r^\dagger)^p.
    \end{align*}
    To see \cref{im:svpRadii2}, notice that since $r'^p=\Omega({m})$, we can assume that $(1+\delta/100)\leq r'^p/10$. This implies,
    \begin{align*}
        (\gamma r)^p &\leq \left(1+\delta/100\right)\left(1+\left(1-\frac{\delta}{2}\right)\frac{2r'^p}{\delta}\right)\\
        &\leq \frac{ r'^p}{10}+\left(1+\delta/100\right)\left(\left(1-\frac{\delta}{2}\right)\frac{2r'^p}{\delta}\right)\\
        & \leq \paren{\frac{\delta}{10}+\paren{1+\frac{\delta}{100}}\paren{2-\delta}}\left(\frac{r'^p}{\delta}\right)\\
        &=\paren{2-\frac{22}{25}\delta-\frac{\delta^2}{100}}\paren{\frac{r'^p}{\delta}}\\
        &< \paren{\frac{2r'^p}{\delta}}\\
        &= (\alpha r^\dagger)^{p}.
    \end{align*}
    For \cref{im:svpRadii3}, use the fact $\gamma^p \leq 1+\delta\cdot \frac{(\sqrt{\gamma'}-1)^2}{2}$ and $\gamma'\geq 1$. Again, since $r'^p=\Omega({m})$ , WLOG we can assume that, $\frac{\delta r'^p}{2}\geq \gamma^p$. Hence we get,
    \begin{align*}
        (\gamma r)^p &\leq \paren{\frac{2r'^p}{\delta}}\paren{\paren{1-\frac{\delta}{2}}\paren{1+\delta\cdot \frac{(\sqrt{\gamma'^p}-1)^2}{2}}}+\gamma^p\\
        &= \paren{\frac{2r'^p}{\delta}} \paren{\paren{1-\delta\sqrt{\gamma'^p}}+\paren{\frac{\delta \gamma'^p}{2}+\frac{\delta^2 \sqrt{\gamma'^p
        }}{4}}-\paren{\frac{\delta(\delta+\delta \gamma'^p)}{4}}}+\gamma^p\\
        &\leq \paren{\frac{2r'^p}{\delta}} \paren{\paren{1-\delta\sqrt{\gamma'^p}} + \frac{\delta \gamma'^p}{2} -\frac{\delta^2}{4}}+\gamma^p\\
        &=(1 - \delta\sqrt{\gamma'^p}) (\alpha r^{\dagger})^p+(\gamma'r)^p- \frac{\delta r'^p}{2}+\gamma^p\\
        &\leq (1 - \delta\sqrt{\gamma'^p}) (\alpha r^{\dagger})^p+(\gamma'r)^p .
    \end{align*}
This concludes the proof of the claim.
\Cref{im:svpRadii1} implies that 
        \begin{align}
        \label{eqn:GZBound}
        G = \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}} \geq \nump{\alpha \Z^{d}, (1-\delta)^{1/p}\alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}.
        \end{align}
        %%%%%%%%%%%%%%
        \Cref{im:svpRadii2,im:svpRadii3} and \cref{eqn:numpKsvp} imply that
        \begin{align*}
        \label{eqn:AZbound}
            A &= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{\alpha}{2}\vec{1}_m}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \notag \\
            &\leq 2 (\gamma r+1) K^m \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\} \\
            &\leq \frac{1}{3^m} 2 (\gamma r+1) \min\{\phi_0,\phi_1\}^{d} \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\}.
        \end{align*}
        For our choice of $d, \dgr r, \delta$, together with \cref{eqn:SvpIntegerGadgetCond}, and the fact that $r = \order{m^{1/p}}$, these imply that for a sufficiently large $m$, $G \geq 2^m A$.
\end{proof}


%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%


\begin{theorem}
    \label{thm:linToSvp}
    For any $p \geq 2+10^{-7}$, there exists a constant $\gamma > 1$ such that for all $n \in \Z^+$, there is a polynomial time randomized Karp reduction from $\lin_\varepsilon$ in $n$ variables and $\order{n}$ equations to $\svp_{p, \gamma}$ in a lattice of rank $\order{n}$.
\end{theorem}

% \adi{Perhaps change $\dgr m$ to $d$ everywhere in the proof.}
\begin{proof} Fix a $p$. We first describe the algorithm, and then show correctness. 

    \textbf{Algorithm.}
%     Fix a $p$, define $\gamma' := \paren{1 + \frac{8\varepsilon}{3}}^{1/p}$.
%     On input a $\lin_\varepsilon$ instance $M \in \F_2^{m \times n},~\vec v \in \F_2^m$, the reduction computes a $\cvp_{p, \gamma'}$ instance $(B', \vec t', r')$ using the algorithm from \cref{thm:LinCvpReduction}.
%     Recall from the proof of \cref{thm:LinCvpReduction} that if this instance is a \yes instance, then $\dist_p(\lat(B'), \vec t') \leq r'$, and if this instance is a no instance then $\dist_p(\lat(B'), \vec t') \geq (\gamma' r')$. 
%     Also recall that by construction, $\rank(\lat(B')) = m$, $\lat(B') \subseteq \Z^m$, $\vec t' \in \lat(B') / 2$ and $\vec t' \in \Z^m$.
%     We claim that by applying the transformation from \cref{lem:cvpToSvp} for a particular choice of efficiently computable parameters $\alpha$, $r$, $\gamma$ and $d$ (to be determined in what follows), the reduction can find a lattice $\lat$ of rank $\order{n}$ that satisfies the conditions in equations \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo}. 
%     Define
%     \begin{equation}
%         \label{eqn:svpGood}
%     G := \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}},
% \end{equation}
%     \begin{align}
%         \label{eqn:svpAnnoying}
%         A &:= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \\ 
%         &\geq \paren{\floor{\gamma r} + 1} \nump{\Z^m, \gamma r, \vec 0} \paren{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}} + \nump{\alpha \Z^{d}, \gamma r, \vec 0} }. \notag
%     \end{align}
%     Notice that $G$ and $A$ are simply the RHS of \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo} respectively. \Cref{eqn:svpGood} and \cref{eqn:cvpToSvpYes} imply that if the input was a \yes instance of $\lin_\varepsilon$, then $$\nump{\lat, r, \vec 0} \geq G.$$
%     Similarly, \cref{eqn:svpAnnoying} and \cref{eqn:cvpToSvpNo} imply that if the input was a \no instance of $\lin_\varepsilon$, then $$\nump{\lat, \gamma r, \vec 0} \leq A.$$
The reduction uses the algorithm from \cref{lem:AGRelation} to compute $(B, \gamma, r, A, G)$. Then it
    % The reduction computes such a lattice, and then 
    samples a prime number $$q \in [\sqrt{AG} / 42,~42\sqrt{AG}],$$
    and uses the algorithm from \cref{lem:svpSparcification2} to get a basis $B'$ of sparse sub-lattice lattice $\lat' \subseteq \lat$ of rank $\order{n}$, and outputs $(B', r)$. The efficiency follows from the efficiency of \cref{lem:AGRelation} and \cref{lem:svpSparcification2}. We now prove correctness. 
    % The three transformations used by the reduction (\cref{thm:LinCvpReduction}, \cref{lem:cvpToSvp} and \cref{lem:svpSparcification2}) are efficient in $n$, therefore reduction is efficient. We now show correctness, and help her choose $\alpha$, $r$, $\gamma$ and $d$.
    % so that the number of ``good" vectors in the \yes case is much larger than the number of ``annoying" vectors in the \no case. 
    % Then the lattice $\lat$ can be sparcified using randomized process from \cref{lem:svpSparcification} to obtain another lattice $\lat''$ of rank $n''$ such that if the input $\lin$ instance was a \yes instance, with high probability at least one good vector of length at least most $r$ survives the sparcification process, and if the input $\lin$ instance was a \no instance, then with high probability all the vectors of length at most $\gamma r$ get killed.
    % In what follows, we first derive the parameters $\alpha$, $r$, $\gamma$ and $\dgr m$. We then continue to describe the action of the oracle following this transformation. 
    % We wish to lower bound the number of good vectors in the \yes case (LHS of \cref{eqn:cvpToSvpYes}) by the LSH of \cref{eqn:SvpIntegerGadgetCond}, 
    % and upper bound the number of annoying vectors in the \no case (LHS of \cref{eqn:cvpToSvpNo}) by the RHS of \cref{eqn:SvpIntegerGadgetCond}.

    % \textbf{Correctness.} 
    % Let $\delta$ be as in \cref{thm:SvpIntegerGadget} for the parameters $(p, \sigma=\gamma'^p)$. Fix $r, \gamma$ such that 
    % $$r^p = \svprval; \quad \quad \gamma^p = \svpgammaval.$$
    % By \cref{lemma:theta0}, for any $\gamma r,~\tau$, there exists a $K > 0$ such that 

    % \begin{align}
    %     \nump{\Z^{m}, \gamma r, \vec 0} &\leq \exp(\tau (\gamma r)^p) \Theta(\tau, \vec 0) \notag \\ 
    %     &= \exp(\tau (\gamma r)^p) \Theta(\tau, 0)^{m} \notag \\ 
    %     &\leq K^{m} && (\because r^p \in \order{m}).
    % \label{eqn:numpKsvp}
    % \end{align}

    % Let $\phi_0, \phi_1$ be the constants from \cref{thm:SvpIntegerGadget} for the particular $p$.
    % Set $$d = \max\left\{ \ceil{\log_{\phi_0}(3K)}, \ceil{\log_{\phi_1}(3K)} \right\} m,$$ and let $\delta,~\dgr r$ be the corresponding constants from that satisfy \cref{eqn:SvpIntegerGadgetCond}.
    % A simple but tedious calculation shows that the following is true. We defer the proof to the appendix. 
    % \begin{restatable}{claim}{claimSvpGadgetParam}
    %     \label{claim:SvpGadgetParameter}
    %     \adi{For any $p,\gamma'$?} If we set 
    %     \begin{align*}
    %     \alpha^p = \svpalphaval;
    %     \quad \quad r^p = \svprval; 
    %     \quad \quad \gamma^p = \svpgammaval;
    % \end{align*}
    % then the following holds. 
    % \begin{enumerate}
    %     \item $\left(r^{p} - 1 - r'^p\right)^{1/p} \geq (1-\delta)^{1/p} (\alpha r^{\dagger})$. \label{im:svpRadii1}
    %     \item $\gamma r \leq \alpha r^{\dagger}$ \label{im:svpRadii2}
    %     \item $\left((\gamma r)^p - (\gamma' r')^p \right)^{1/p}\leq (1 - \delta\sqrt{\gamma'^p})^{1/p} (\alpha r^{\dagger})$ \label{im:svpRadii3}
    % \end{enumerate}
    % \end{restatable}
    
    % \Cref{im:svpRadii1} implies that 
    %     \begin{align}
    %     \label{eqn:GZBound}
    %     G = \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}} \geq \nump{\alpha \Z^{d}, (1-\delta)^{1/p}\alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}.
    %     \end{align}
    %     %%%%%%%%%%%%%%
    %     \Cref{im:svpRadii2,im:svpRadii3} and \cref{eqn:numpKsvp} imply that
    %     \begin{align*}
    %     \label{eqn:AZbound}
    %         A &= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{\alpha}{2}\vec{1}_m}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \notag \\
    %         &\leq 2 (\gamma r+1) K^m \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\} \\
    %         &\leq \frac{1}{3^m} 2 (\gamma r+1) \min\{\phi_0,\phi_1\}^{d} \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\}.
    %     \end{align*}
    %     For our choice of $d, \dgr r, \delta$, together with \cref{eqn:SvpIntegerGadgetCond}, and the fact that $r = \order{m^{1/p}}$, these imply that for a sufficiently large $m$, $G \geq 2^m A$.
    \textbf{Correctness.} 
        We bound the probability of a lattice vector of a particular length making it into the sparse sub-lattice $\lat'$ lattice. 
        Suppose that the input was a $\yes$ instance of $\lin_\varepsilon$. Let $\mathcal{S}$ be the set of {\em good} lattice vectors in $\lat$ of length at most $r$. 
        % These are distinct vectors of the form $\vec v_1 \oplus \vec v_2 \oplus 1$, where $\vec v_1 \in \lat(B') - \vec t' ,~\vec v_2 \in \alpha \Z^{d} - \frac{\alpha}{2}\vec 1_{d}$, and therefore they are linearly independent. Then 
        These are distinct lattice vectors such that their last coordinates are all $1$. Therefore, they are all primitive and hence pairwise linearly independent. It is also clear that $r \leq q \lambda_1^{(p)}(\lat)$. Then,
        $$\abs{\mathcal{S}} \geq G \implies \frac{q}{\abs{\mathcal{S}}} \leq {42} \cdot \sqrt{\frac{A}{G}} \in \order{-2^{m/2}}.$$
        Therefore by the lower bound in \cref{lem:svpSparcification2}, $(B', r)$ is a \yes instance of $\svp_{p, \gamma}$ except with an exponentially small probability. Next, suppose that the input was a \no instance of $\lin_\varepsilon$. Let $\mathcal{S}$ be the set of {\em annoying} vectors of length {\em at most} $\gamma r$. We have that $\abs{\mathcal{S}} \leq A$, and hence the number of linearly independent vectors in $\mathcal{S}$ of length at most $\gamma r$ is at most $A$.
        Additionally, we claim that in this case $\gamma r \leq q \lambda_1^{(p)}(\lat)$. Too see this, suppose $\gamma r > q \lambda_1^{(p)}(\lat)$ for contradiction. This implies that $\lambda_1^{(p)}(\lat) < \frac{\gamma r}{q} < \frac{\gamma r}{A}$, because $q > A$. Let $\vec v \in \lat$ be such that $\norm{\vec v}_p = \lambda_1^{(p)}(\lat)$. Then, $\{ -A \vec v, \ldots A\vec v \}$ are $2A$ vectors of length at most $\gamma r$, contradicting the fact that $\nump{\lat, \gamma r, \vec 0} \leq A$.  
        Therefore, 
        $$ \frac{\abs{\mathcal{S}}}{q} \leq 42 \cdot \sqrt{\frac{A}{G}} \in \order{2^{-m/2}},$$
        and by the upper bound in \cref{lem:svpSparcification2}, $(B', r)$ is a \no instance of $\svp_{p, \gamma}$ except with an exponentially small probability. \qedhere

    % Together with \cref{eqn:numpthetasvp}, \cref{eqn:SvpIntegerGadgetCond} and the fact that $\gamma r = \order{r'} = \order{n}$ imply that for a sufficiently large $n$, $G \geq 2^{n'}A$. 

    % We now continue with the action of the reduction algorithm. 
    % Define $P := 10\sqrt{AG}$. The reduction does the following $\ell := \ceil{100n'\log P}$ times. It samples a prime number $q$ in the range $[10 P \log P,~20 P \log P]$, and uses the algorithm from \cref{lem:svpSparcification2} to obtain (a basis of) a sub-lattice $\lat''$ of rank $n' + d + 1 = \order{n}$.
    % Then it uses its $\svp_{p, \gamma}$ oracle to check if $\lambda_1^{(p)}(\lat'') \leq r$. It outputs \yes iff the oracle returns \yes more than $\delta \ell$ times, where
    % \[ \delta := \frac{P}{20q} - \frac{P^2}{200q^2} \geq \frac{1}{100 \log P}. \]

    % Suppose that the input $\lin_\varepsilon$ instance was a \yes instance. Then, $\lat'$ has at least $G$ vectors of length at most $r$. By the construction in \cref{eqn:cvpToSvpBasis}, these are vectors with their last coordinates as $1$, and thus are all primitive vectors. By \cref{lem:svpSparcification2}, 
    % \begin{align*}
    %     \Pr \left[ \lambda_1^{(p)}(\lat'') \leq r \right] &\geq 2 \delta.
    % \end{align*}
    % Therefore, the reduction outputs \yes except with probability at most $\exp\paren{-\Omega(d)}$ by Chernoff-Hoeffding bound. 

    % Next suppose that the input $\lin_\varepsilon$ instance was a \no instance. Then, $\lat'$ has at most $A$ vectors of length at most $\gamma r$, and thus at most $A$ {\em primitive} vectors of that length. Again by \cref{lem:svpSparcification},
    % \begin{align*}
    %     \Pr \left[ \lambda_1^{(p)}(\lat'') \leq r \right] &\leq \frac{A}{q} \leq \frac{\delta}{2}.
    % \end{align*}
    % Therefore, the reduction outputs \no except with probability at most $\exp\paren{-\Omega(d)}$, again by Chernoff-Hoeffding bound.

\end{proof}

Together with \cref{cor:linEthHard}, we get the following theorem.

\thmsvpethhard*


% \begin{theorem}
% \label{thm:mintoagsvp}
% Suppose for $p \in [1, \infty)$, there exist constants $\alpha_G \geq \alpha_A > 0$, $\nu_0, \nu_1 > 1$, and a family of efficiently computable lattice target pairs\footnote{By an efficiently computable lattice gadget, we mean that there is a (randomized) algorithm that given an input $n$, outputs $(\dgr{B}_{n}, \vec t^{\dagger}_n)$ in time $\poly(n)$. Similarly, by efficiently computable functions, we mean that there is a (randomized) algorithm that approximates the function to within a $2^{o(n)}$ factor in $\poly(n)$ time, where $n$ is the length of its input.} $\set{(\dgr{B}_{\dgr{n}}, \dgr{\vec{t}_{\dgr n}})}_{\dgr{n} = 1}^{\infty}$ for each $\dgr{n}$ such that $\rank(\cL(B_{\dgr{n}})) = \dgr{n}$, $\dgr{\vec t}_{\dgr{n}} \in \spn{\dgr{B}_{\dgr{n}}}$, $\forall l \in 2\Z, l \dgr{\vec t}_{\dgr n} \in \lat(\dgr B_{\dgr n})$, and
% \begin{equation}
%     \label{eqn:svpgadgetcondreq}
%     \nump{\cL(B_{\dgr{n}}), \alpha_G + o(1), \dgr{\vec{t}}_{\dgr{n}}} \geq \max\left\{ \nu_0^{\dgr{n} - o(1)} \numpo{\dgr{\cL}_{\dgr{n}}, 1, \vec{0}}, \nu_1^{\dgr{n} - o(1)} \numpo{\dgr{\cL}_{\dgr{n}}, \alpha_A, \dgr{\vec{t}_n}} \right\}.
% \end{equation}
% Further, suppose that each term in the above inequality is efficiently computable.
% Then for all constants $ C > 1, \varepsilon > 0$, there exists constant $\gamma > 1$ and $G(n), A(n)$ such that $G(n) \geq 2^n A(n)$ such that there is a (randomized) polynomial time Karp reduction from $\lin_{\varepsilon}$ in $n$ variables to $(A, G)$-$\svp_{p, \gamma, r}$ in rank $Cn$ for all sufficiently large $n$.
% \end{theorem}

% \begin{proof}
    
% \end{proof}




==> svp_focs.tex <==
In this section we show a reduction from $\sat$ in $n$ variables to $\svp_{p, \gamma}$ in a lattice of rank $\order{n}$. 
We do this by a reduction from $\cvp_{p, \gamma'}$ for a constant $\gamma'$ (an instance obtained in \cref{sec:cvp_hard}) to $\svp_{p, \gamma}$ for a constant $\gamma$. 
The result then follows from combining the reduction from $\sat$ to $\lin$ in \cref{thm:satToLinRed}, and from $\lin$ to $\cvp$ in \cref{thm:LinCvpReduction}. 
We first show that a (family of) locally dense lattice gadget-target pairs with certain properties exist, which will be used in our reduction.
In \cref{ssec:all_half_target} we show that for $p \geq 2 + 10^{-7}$, the integer lattice with the all half vector as the target is sufficient to show the reduction. We are, however, unable to prove that this works for all $p > 2$. We conjecture that this is in fact the case, and leave it as an interesting mathematical question for future work. 
In \cref{ssec:locally_dense_lattices}, we show that for all $p > 2, d \in \Z^+$, we can find a vector in $\Q^d$ that, along with the integer lattice, is sufficient for our reduction. 

\subsection{Locally Dense Integer Gadget with the all-half target}
\label{ssec:all_half_target}


We wish to show that in the integer lattice $\Z^n$, there are exponentially more vectors close to $\frac{1}{2}\vec 1_n$ than the number of {\em short} vectors. The following property of the theta function will be useful. 

\begin{lemma}
    \label{lem:thetaProp}
    For every $p \geq 2+10^{-7}$, there exists a $\tau > 0$ such that 
    \begin{equation}
        \label{eqn:thetaProp}
        \Theta_p(\tau, 0) < \Theta_p(\tau, 1/2). 
    \end{equation}
    % Furthermore, $\tau$ can be efficiently computed from $p$.
\end{lemma}

\begin{proof}
% \adi{To be revised thoroughly.}

From the definition, 
\[\Theta_p(\tau,0) = \sum_{z \in \Z} e^{-\tau|z|^p} = 1+ 2 \sum_{z =1}^{\infty} e^{-\tau\cdot z^p},\]
and 
\[\Theta_p(\tau,1/2) = \sum_{z \in \Z} e^{-\tau|z-1/2|^p} =  2 \sum_{z =1}^{\infty} e^{-\tau \cdot (z-1/2)^p}.\]
      %%%%%%%%%%%%%%%%%%%
      %%%%%%%%%%%%%%%%%%%
Define 
\[ A_z(p, \tau) := e^{-\tau (z - 1/2)^p} - e^{-\tau z^p}, \]
% \[ \Delta(p,\tau) := \sum_{z = 1}^{\infty} A_z(p, \tau) = \sum_{z = 1}^{\infty} \paren{ e^{-\tau (z - 1/2)^p} - e^{-\tau z^p} }. \]
% and
\[
S_n(p,\tau) := \sum_{z=1}^{n} A_z(p,\tau)
\]
The condition $\Theta_p(\tau,0)<\Theta_p(\tau,1/2)$ is equivalent to,\[S_\infty(p,\tau)>0.5\]
Observe that $\forall z \geq 1,~A_z > 0$. It is enough to show that for $p \geq 2.001$, there exists $n \in \N, \tau>0$ such that $S_n(p,\tau) > 1/2.$ 
Also,
\[ \frac{\partial A_z(p, \tau)}{\partial p} = -\tau\cdot \left( e^{-\tau \cdot (z-0.5)^p} (z-0.5)^p \ln(z-0.5) - e^{-\tau\cdot z^p} z^p \ln z \right) \]


      
\textbf{Suppose $p\geq 2.2$.} We claim that in this case, $\exists \tau > 0$ such that $\forall p \geq 2.2,~S_1(p, \tau) = A_1(p, \tau) > 1/2.$ Differentiating $A_1(p, \tau)$ with respect to $p$, we see that
\[
\frac{\partial A_1(p, \tau)}{\partial p} = \tau e^{-\tau (1/2)^p} \cdot (1/2)^p \cdot \ln(2) >0.
\]
This implies that $A_1(p, \tau)$ is increasing with respect to $p$. Therefore it suffices to find a $\tau>0$ such that $A_1(\tau,2.2)>0.5$. 
Conveniently, we find that for $\tau = 1.949$, $~A_1(2.2, 1.949) > 0.5$\footnote{This $\tau$ is chosen such that it is close to the maximizer of $A_1(\tau, 2.2).$}. 
% \tau=\frac{2^{2.2}\ \ln(2^{2.2})}{2^{2.2}-1}

\textbf{Suppose $p \in [2.001, 2.2)$.}
% \footnote{From here on, since the proof is somewhat computational, the reader may use the following script to verify the work on \href{https://colab.research.google.com/drive/1T-4dKo1LHMgMow1UGGgBRdY-2aslCjq1?usp=sharing}{Colab}. Additionally, a \href{https://www.desmos.com/calculator/i3tzezgkzq}{Desmos} link with a plot of the feasible region is available.} 
We will truncate the series $S_{\infty}$ to the first ten terms and fix $\tau = \tau_0 := 0.89$. Define
\[h(p) = S_{10}(p,0.89) = \sum_{z=1}^{10} e^{- \tau_0 \cdot (z-0.5)^p}- e^{-\tau_0 \cdot z^p}.\]
We claim that for $2.001 \leq p <2.2$, $h(p)>0.5$. To see that, consider the derivatives with respect to $p$,
\[
h'(p) = \sum_{z=1}^{10} -\tau_0\cdot \left( e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p \ln(z-0.5) - e^{-\tau_0\cdot z^p} z^p \ln z \right)
\;,\]
and, 
\begin{align}
h''(p) = \tau_0^2\cdot\sum_{z=1}^{10}  \left( e^{- \tau_0 \cdot(z-0.5)^p} (z-0.5)^{2p} (\ln(z-0.5))^2 \right)+\tau_0\sum_{z= 1}^{10}\left( e^{-\tau_0\cdot z^p} z^p (\ln z )^2\right) \notag \\
-\tau_0^2\sum_{z=1}^{10}\left( e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 \right) -\tau_0\cdot \sum_{z=1}^{10} \left( e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2\right).
\label{eqn:uglyproof1}
\end{align}
We wish to find an $L>0$ such that if $2.001\leq p < 2.2$, then $-L\leq h''(p)$. For that, we collect all the negative terms from \cref{eqn:uglyproof1} and get the following bound,
\[h''(p)>-\tau_0^2 \left(\sum_{z=2}^{10} e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 \right)-\tau_0\left( \sum_{z=2}^{10} e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2\right) -\frac{\tau_0 e^{-\tau_0/2^p} \cdot (\ln{2})^2}{2^p}.\] 
Since $2<p\leq 2.2$, using the fact that for $x>1$ and 
\begin{align}
    e^{-\tau_0 \cdot x^p}<e^{-\tau_0 \cdot x^2} \text{ and } x^{2p}<x^{5} \label{eqn:weirdineq1} ,\\
     e^{-\tau_0 \cdot x^p}<e^{-\tau_0 \cdot x^2} \text{ and } x^{p}<x^{3} \label{eqn:weirdineq2}.
\end{align}
we get that for $z\geq2$,
\begin{align*}
   % z^{2p}<z^5,e^{-\tau_0 \cdot z^p}\leq e^{-\tau_0\cdot z^2}\implies 
   e^{-\tau_0 \cdot z^p} z^{2p} (\ln z)^2 &\leq e^{-\tau_0 \cdot z^2} z^{5}(\ln z)^2; && \text{(from \cref{eqn:weirdineq1})}\\
    % (z-0.5)^{p}<(z-0.5)^3,e^{-\tau_0 \cdot (z-0.5)^p}\leq e^{-\tau_0\cdot (z-0.5)^2}\implies
    e^{-\tau_0 \cdot (z-0.5)^p} (z-0.5)^p (\ln(z-0.5))^2 & \leq e^{-\tau_0 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2; && \text{(from \cref{eqn:weirdineq2})}\\
    \frac{e^{-\tau_0 / 2^p}  (\ln 2)^2}{2^p} &\leq \frac{e^{-\tau_0/8} \cdot (\ln{2})^2}{4}.
\end{align*}
This implies that for all $2.001\leq p \leq 2.2$,
\begin{align*}
h''(p)&>\:-\tau_0^2 \left(\sum_{z=2}^{10}  e^{-\tau_0 \cdot z^2} z^{5} (\ln z)^2 \right) -\tau_0\left( \sum_{z=2}^{10} e^{-\tau_0 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2\right) -\frac{\tau_0 e^{-\tau_0/8} \cdot (\ln{2})^2}{4} \\ & >\;(-0.64).
\end{align*}
%%%%%%


%%%%%%
Notice that for any finite $z \in \Z$, $A_z(p, \tau)$ is a smooth function. Therefore a finite truncation of the sum $S_{\infty}$ is a smooth function. Hence, we can use Taylor's theorem \cite[Theorem 6.4.1]{bartle} to bound the values in the intervals $2.001 \leq p \leq 2.1 $ and $2.1 \leq p \leq 2.2$. 
Let $\Delta = (p-2.001)$. By Taylor's theorem, for any $p \in[2.001,2.1]$, there exists a $p'\in[2.001, p]$ such that,  
$$h(p) = h(2.001)+ h'(2.001)\cdot \Delta+\frac{h''(p')\cdot\Delta^2}{2} \:.$$ 
We have that $h(2.001)\geq 0.50000971 >0.5$ and $h'(2.001)\geq 0.067056759$. Since $h'(2.001)>0$, and $\Delta \in [0,0.099]$ then
using the fact that $h''(p')>-0.64$ we get that,
$$h(p)\geq\min_{\Delta \in[0,0.099]}\left\{h(2.001)+h'(2.001)\cdot\Delta-\frac{ (0.64)\Delta^2}{2} \right\} \:.$$
Let, $$q(\Delta)= h(2.001)+h'(2.001)\cdot\Delta-\frac{(0.64) \Delta^2}{2} \:.$$
Since $q $ is an inverted parabola, the minimum on the interval $[0,0.099]$ must be attained at one of the end points of the interval and we get that $q(0)=h(2.001)>0.5$ and $q(0.099)\geq  0.5035>0.5$.
Similarly since $h(2.1)\geq 0.50623643$ and $h'(2.1)\geq 0.05875258>0$ for all $p\in[2.1,2.2]$ we get that,
\begin{align*}
h(p)&\geq \min_{\Delta \in[0,0.1]}\left\{h(2.1)+h'(2.1)\cdot\Delta-\frac{ (0.64)\Delta^2}{2} \right\} \: .\end{align*}
Now again let, 
$$q_1(\Delta)= h(2.1)+h'(2.1)\cdot\Delta-\frac{(0.64) \Delta^2}{2} \:.$$
Again, since $q_1$ is an inverted parabola, we get that for all $p\in[2.1,2.2]$, $h(p)\geq \min \left\{q_1(0), q_1(0.1)\right\}$. Since $q_1(0)=h(2.1)>0.5$ and $q_1(0.1)\geq 0.5089>0.5$, we get that $h(p)>0.5$ for all $p \in [2.001,2.2]$.

\textbf{Suppose} $p \in [2+10^{-7}, 2.001)$. Take $\tau_1=0.162665$ and $h(p) = S_{11}(p, \tau_1)$.
Using an argument along similar lines as that in the previous case, we get that for all $2+10^{-7}\leq p \leq 2.001$,
\begin{align*}
h''(p)&>\:-\tau_1^2 \left(\sum_{z=2}^{11}  e^{-\tau_1 \cdot z^2} z^{5} (\ln z)^2 \right) -\tau_1\left( \sum_{z=2}^{11} e^{-\tau_1 \cdot (z-0.5)^2} (z-0.5)^{3} (\ln(z-0.5))^2\right) -\frac{\tau_1 e^{-\tau_1/8} \cdot (\ln{2})^2}{4} \\ & >\;(-16.5).
\end{align*}

This time, we have that $h(2+10^{-7})\geq 0.50000000051525>0.5$ and $h'(2+10^{-7})\geq0.009104222964$. Therefore, by Taylor's Theorem we get that for all $p\in [2+10^{-7},2.001]$,
\begin{align*}
    h(p) &\geq  \min_{\Delta \in[0,0.001]}\left\{h(2+10^{-7})+h'(2+10^{-7})\cdot\Delta-\frac{ (16.5)\Delta^2}{2} \right\}\\
    &\geq \min\left\{h(2+10^{-7}), 0.5000008\right\}\\
    &>0.5
\end{align*}
\end{proof}


\begin{theorem}
    \label{thm:SvpIntegerGadget}
    For any $p \geq 2+10^{-7},~\sigma > 1$, there exists constants $\delta \in (0, 1/2)$, $\phi_0, \phi_1 > 1$ and $C_r>0$, such that for any $n \in \Z^+$, if $r :=C_r \cdot {n^{1/p}}$ then the following holds for the integer lattice. 
    \begin{align}
        \nump{\Z^{n}, (1-\delta)^{1/p} r, \frac{1}{2}\vec{1}_{n}} \geq \max\bigg\{ &\phi_0^{n - o(n)} \nump{\Z^{n}, r, \vec{0}}, \notag \\
        &\phi_1^{n - o(n)} \nump{\Z^{n}, (1-\delta\sqrt{\sigma})^{1/p} r, \frac{1}{2} \vec{1}_{n}} \bigg\}.
        \label{eqn:SvpIntegerGadgetCond}
    \end{align} 
     The constants $\delta, \phi_0, \phi_1, C_r$ only depend  upon $p$ and can be efficiently computed with required precision, from $p$. 
\end{theorem}

% \adi{To be revised thoroughly.}   
% \adi{Change $\dgr m$ to $n$, $\dgr r$ to $r$.}
% \adi{Use appropriate macros and restatables instead of rewriting.}
% \adi{Equation spacing is fucked up.}
% \adi{Write that the constants can be estimated efficiently, reformulate that theorem properly and check the quatification.}

\begin{proof}
Fix any $p$ and $\sigma$. Fix $\tau > 0$ as in \cref{lem:thetaProp}. Then define 
$$\rho:=\frac{\Theta_p(\tau,1/2)}{\Theta_p(\tau,0)}>1.$$ 
Notice that the precision to which we would approximate $\rho$ would be independent of the input size, so such a $\rho$ is efficiently computable in constant time. 
For a $\delta \in (0, 1/2)$ to be determined in what follows, fix 
$$C_r := \frac{\mu_p(\tau,1/2)^{1/p}}{(1-\delta)^{1/p}}.$$
 By \cref{thm:theta_gives_good_approx}, there exists a constant $C^*>0$ such that,

\begin{equation}
\label{eq:bd1}
\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}} \geq \exp\left(-C^* \sqrt{n}\right)\cdot \exp(\tau n \cdot \mu_p(\tau,1/2))\cdot \Theta_p(\tau , 1/2)^{n}.
\end{equation}

By \cref{lemma:theta0}, 
\begin{equation}
\label{eq:bd2}
\nump{\Z^{n},r,\vec{0}} \leq \exp\paren{\tau \cdot\frac{n ~\mu_p(\tau,1/2)}{1-\delta}}\cdot \Theta_p(\tau,0)^{n}.
\end{equation}
% \[N_p(2\Z^{m^\dagger},r^\dagger,0)\leq \exp\paren{\tau \cdot\frac{m^\dagger \cdot \mu_p(\tau,1/2)}{1-\delta}}\cdot \Theta_p(\tau,0)^{m^\dagger}\]
From \cref{eq:bd1,eq:bd2}, we get that 
\[\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}}}{\nump{\Z^{n},r,\vec{0}}} \geq \rho^{n} \cdot \exp\left(-C_r^p\tau\delta n -o(n)\right).\]
Because $\rho>1$, we can fix $\delta>0$ such that,
$$\delta < \frac{\log \rho}{\tau \mu_p(\tau, 1/2) + \log \rho},$$
which implies that $\rho \cdot \exp(-\tau \delta C_r^p)>1$. 
Then set $\phi_0:=\rho \cdot \exp(-\tau \delta C_r^p)$. This implies that, 
$$\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}}}{\nump{\Z^{n},r, \vec{0}}} \geq \phi_0^{n -o(n)}.$$

For the second inequality, again use \cref{lemma:theta0} to get,
\begin{equation}
\label{eq:bd3}
N_p\left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}\right)\leq \Theta_p(\tau,1/2)^{n} \cdot \exp\paren{\tau \cdot n C_r^p \cdot (1-\delta\sqrt{\sigma})}.
\end{equation}
Then set  $\phi_1:=\exp \paren{\tau\delta C_r^p\cdot(\sqrt{\sigma}-1)}>1$ which implies,
\[\frac{N_p\left(\Z^{n},(1-\delta)^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n}\right)}{N_p \left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\frac{1}{2}\vec{1}_{n} \right)}\geq \exp \paren{\tau\delta n C_r^p\cdot(\sqrt{\sigma}-1) -o(n)}=\phi_1^{n-o(n)}. \]
\end{proof}




We conjecture the following.
\begin{conjecture}
\label{conj:the_conjecture}
    For every $p>2$ there exists a $\tau>0$, such that,
    \[\Theta_p(\tau,1/2)>\Theta_p(\tau,0)\]
\end{conjecture}

In the following section, we are able to bypass this mathematical bottleneck by showing that for any $p > 2$, there exists a target that works with our reduction. 


\subsection{Locally Dense Integer Gadget}
\label{ssec:locally_dense_lattices}

We show that for all $n \in \Z^+$, there exists a target $\vec t \in \spn(\Z^n)$ of the form $t \cdot \vec 1_{n}$ such that there are exponentially more integer points around $\vec t$ than around $2\ell \vec t$, for any $\ell \in \Z$.
We will use the following property of the theta function.

\begin{lemma}
\label{lem:existt}
For any $p > 2$ and $\tau \geq 1 - 1/p$, there exists a $z\in\Z$ such that,
\[
\Theta_p \left(\tau, \frac{1}{2^z}\right) > \Theta_p\left(\tau, 0\right).
\]
\end{lemma}
\begin{proof}
Notice that $\exp(-\tau |t|^p)$ is twice differentiable at $t = 0$ for $p > 2$, with first and second derivative both zero. Therefore, we have that,
\[
\frac{\partial}{\partial t} \Theta_p(\tau, t) \Big|_{t=0} = 0,
\]
and
\[
\frac{\partial^2}{\partial t^2} \Theta_p(\tau, t) \Big|_{t=0} = p\tau \sum_{z \in \mathbb{Z}} \exp(-\tau |z|^p) |z|^{p-2} (p\tau |z|^p - (p-1)).
\] 

For $\tau \geq 1 - 1/p$, all of the summands in the above expression of the double derivative are non-negative, which implies $0$ is a local minimum of the function $t \mapsto \Theta_p(\tau, t)$. Therefore, for a sufficiently large $z\in\Z$, $1/2^z$ lies in a small enough neighborhood around 0 so that $\Theta_p(\tau,1/2^z) > \Theta_p(\tau, 0)$, as needed.
\end{proof}
%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%
\begin{lemma}
\label{newidea}For any $p>2$ , there exists a $t\in[0,1/2)$
such that for all $\cl \in \Z$, 
\begin{equation}\label{cl22}
\Theta_p\paren{1,t} \geq \Theta_p\paren{1,\cl t}.
\end{equation}
Moreover, if $\cl \in 2\Z$ then
\begin{equation}\label{cl11}
\Theta_p\paren{1,t} > \Theta_p\paren{1,\cl t}
\end{equation}
\end{lemma}

\begin{proof}
By \cref{lem:existt}, there exists a $z$ such that
\[\Theta_p \left(1, \frac{1}{2^z}\right) > \Theta_p\left(1, 0\right).\]
Set $t_0=1/2^z$, for such a $z$.
Define 
\begin{align*}
T &:= \set{\Theta_p\paren{1,\cl t_0} \;\mid \cl\in \Z} \\
&=\set{\Theta_p\paren{1,\cl t_0} \;\mid \cl\in [0,2^z-1]} && (\because 2^z \cdot t_0 \in \Z).
\end{align*}
 
Now let $\Theta_{\max}$ be the maximal element of $T$, and define
 \[M:=\left\{i \;\mid i\in[0,2^{z}-1], \Theta_p\paren{1,i t_0}= \Theta_{\max}\right\}\]
 
Let $k \in M$ be such that the highest power of 2 divides it (i.e., $k$ has the highest $2$-adic valuation (\cref{def:padicval}) among all elements in $M$). 
Note that $k \in M$ implies that $\Theta_p(1, k t_0)\geq \Theta_p(1,t_0)$, which implies that $k$ cannot be $0$. We claim that $k \cdot t_0$ satisfies the required conditions. \Cref{cl22} follows by definition of $M$.
We prove \cref{cl11} by contradiction. Suppose there exists some \( j \in \mathbb{Z} \) such that  
\[ \Theta_p(1, k t_0) = \Theta_p(1, 2j \cdot k t_0). \]  
This implies that  
\[
k' = (2j \cdot k \mod 2^z) \in M.
\]  
However, this would mean that the 2-adic valuation of \( k' \) is strictly greater than that of \( k \), contradicting the choice of \( k \) as the element in \( M \) with the highest 2-adic valuation.
\end{proof}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{theorem}
    \label{thm:SvpIntegerGadget_new}
    For any $p > 2,~\sigma > 1$, there exists constants $t>0,\delta \in (0, 1/2)$, $\phi_0, \phi_1 > 1$ and $C_r>0$, such that for any $n \in \Z^+$,  $\cl_0 \in 2\Z $ and $\cl_1 \in \Z$, if $r :=C_r \cdot {n^{1/p}}$ and $\vec{t}=t\cdot \vec{1}_n$ then the following holds for the integer lattice. 
    \begin{align}
        \nump{\Z^{n}, (1-\delta)^{1/p} r, \vec{t}} \geq \max\bigg\{ &\phi_0^{n - o(n)} \nump{\Z^{n}, r, \cl_0 \cdot \vec{t}}, \notag \\
        &\phi_1^{n - o(n)} \nump{\Z^{n}, (1-\delta\sqrt{\sigma})^{1/p} r, \cl_1 \cdot \vec{t}} \bigg\}.
        \label{eqn:SvpIntegerGadgetCond_new}
    \end{align} 
     The constants $\delta, \phi_0, \phi_1, C_r$ and $t$ only depend  upon $p$ and can be efficiently computed with required precision, from $p$. Moreover, if $p \geq 2 + 10^{-7}$ then $t = 1/2$ suffices. 
\end{theorem}

% \adi{To be revised thoroughly.}   
% \adi{Change $\dgr m$ to $n$, $\dgr r$ to $r$.}
% \adi{Use appropriate macros and restatables instead of rewriting.}
% \adi{Equation spacing is fucked up.}
% \adi{Write that the constants can be estimated efficiently, reformulate that theorem properly and check the quatification.}

\begin{proof}
Fix any $p$ and $\sigma$. Fix $t$ as in \cref{newidea}. Then define 
$$\rho:=\min_{\cl_0\in 2 \Z}\left\{\frac{\Theta_p(1,t)}{\Theta_p(1,\cl_0 t)}\right\}>1.$$ 
Notice that the precision to which we would approximate $\rho$ would be independent of the input size, so such a $\rho$ is efficiently computable in constant time. 
For a $\delta \in (0, 1/2)$ to be determined in what follows, fix 
$$C_r := \frac{\mu_p(1,t)^{1/p}}{(1-\delta)^{1/p}}.$$
 By \cref{thm:theta_gives_good_approx}, there exists a constant $C^*>0$ such that,

\begin{equation}
\label{eq:bd1_new}
\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\vec{t}} \geq \exp\left(-C^* \sqrt{n}\right)\cdot \exp( n \cdot \mu_p(1,t))\cdot \Theta_p(1, t)^{n}.
\end{equation}

For any $\cl_0 \in 2\Z$ by using \cref{lemma:theta0} we get, 
\begin{equation}
\label{eq:bd2_new}
\nump{\Z^{n},r,\cl_0\cdot \vec{t}} \leq \exp\paren{\frac{n \cdot\mu_p(1,t)}{1-\delta}}\cdot \Theta_p(1,\cl_0 t)^{n}.
\end{equation}
% \[N_p(2\Z^{m^\dagger},r^\dagger,0)\leq \exp\paren{\tau \cdot\frac{m^\dagger \cdot \mu_p(\tau,1/2)}{1-\delta}}\cdot \Theta_p(\tau,0)^{m^\dagger}\]
From \cref{eq:bd1_new,eq:bd2_new}, we get that 
\[\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\vec{t}}}{\nump{\Z^{n},r,\cl_0 \cdot \vec{t}}} \geq \rho^{n} \cdot \exp\left(-C_r^p\delta n -o(n)\right).\]
Because $\rho>1$, we can fix $\delta>0$ such that,
$$\delta < \frac{\log \rho}{ \mu_p(1, t) + \log \rho},$$
which implies that $\rho \cdot \exp(- \delta C_r^p)>1$. 
Then set $\phi_0:=\rho \cdot \exp(- \delta C_r^p)$. This implies that for all $\cl_0 \in 2\Z$, 
$$\frac{\nump{\Z^{n},(1-\delta)^{1/p}\cdot r,\vec{t}}}{\nump{\Z^{n},r, \cl_0\cdot \vec{t}}} \geq \phi_0^{n -o(n)}.$$

For the second inequality, again use \cref{lemma:theta0} to get for any $\cl_1 \in \Z$,
\begin{equation}
\label{eq:bd3_new}
N_p\left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\;\cl_1 \cdot \vec{t}\right)\leq \Theta_p(1,\cl_1 t)^{n} \cdot \exp\paren{ n C_r^p \cdot (1-\delta\sqrt{\sigma})}.
\end{equation}
Then set  $\phi_1:=\exp \paren{\delta C_r^p\cdot(\sqrt{\sigma}-1)}>1$ which implies,
\[\frac{N_p\left(\Z^{n},(1-\delta)^{1/p}\cdot r,\vec{t}\right)}{N_p \left(\Z^{ n},(1-\delta\sqrt{\sigma})^{1/p}\cdot r,\; \cl_1 \cdot \vec{t}\right)}\geq \exp \paren{\delta n C_r^p\cdot(\sqrt{\sigma}-1) -o(n)}=\phi_1^{n-o(n)}. \]

Additionally, from \cref{thm:SvpIntegerGadget}, it follows that if $p \geq 2 + 10^{-7}$ then the theorem follows with $t = 1/2$, with the respective constants $\rho, \delta, \phi_0, \phi_1$ and $C_r$.
\end{proof}




\subsection{From \texorpdfstring{$\lin_\varepsilon$ to $\svp_{p, \gamma}$}{lin to svp}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
In the following, we  start with a $\cvp_{p, \gamma'}$ instance with the special property that twice the target vector is in the lattice, and find a lattice $\cL$ and a parameter $r$ such that the number of vectors in $\cL$ of length at most $r$ are $2^{\Omega(n)}$ times more for a YES instance than for a NO instance. 
\begin{lemma}
    \label{lem:cvpToSvp}
    For any $p \in [1, \infty)$, suppose $(B', \vec t', r')$ is a $\cvp_{p, \gamma'}$ instance, such that $B' \in \Z^{m \times m'}, \vec t' \in \lat(B') / 2$ and $\vec t' \in \Z^m$. Then for any $d \in \Z^+ $, given a lattice $\ldgr\subseteq \R^d$ with basis $B^\dagger \in \R^{d\times d'}$, and a target $\tdgr \in \R^d$, there exists an efficiently computable matrix $B$ that generates a lattice $\lat(B)$ in $m + d + 1$ dimensions such that for any constants $\gamma'>1$ and any radii $r_G$,$r_A$,
    \begin{enumerate}
        \item If $\di_p\paren{\vec{t}',\cL(B')}\leq r'$  then,
        \begin{equation}
            \label{eqn:cvpToSvpYes}
        \nump{\lat, r_G, \vec 0} \geq \nump{\ldgr, (r_G^{p} - 1 - r'^p)^{1/p},\tdgr},
    \end{equation}
        \item If  $\di_p\paren{\vec{t}',\cL(B')}> \gamma'r'$ then,
        \begin{align}
            \label{eqn:cvpToSvpNo}
        \nump{\lat, r_A, \vec 0} \leq(r_A +4) \cdot \nump{\Z^m, r_A, \vec 0} \cdot \bigg(&\max_{\cl_1 \in \Z}\left\{\nump{\ldgr,~(r_A^p - (\gamma' r')^p)^{1/p}, \cl_1\cdot \tdgr} \right\} + \notag\\ 
        &\max_{\cl_0 \in 2\Z}\left\{  \nump{\ldgr, r_A, \cl_0 \cdot \vec{t}^\dagger} \right\}\bigg).
    \end{align}
    \end{enumerate}
\end{lemma}

\begin{proof}
% \dnote{The input is given in terms of the generating set. Also, $B$ will define the generating set of $\cL$.}
    % Let $B'$ be a basis for $\lat'$.
    
    Define
    \begin{equation}
        \label{eqn:cvpToSvpBasis}
    B := \begin{pmatrix}
        B' & 0 & -\vec t' \\
        0 & \dgr{B} & - \vec{t}^{\dagger} \\
        0 & 0 & 1
    \end{pmatrix}. 
    \end{equation}
    Then $\lat = \lat(B)$ is a lattice in $m + d + 1$ dimensions, and $B$ is clearly efficiently computable. 
    Suppose that the input $\cvp_{p, \gamma'}$ instance was a \yes instance. This implies that $\dist(\cL', \vec t') \leq r'$. Then $\exists \vec x \in \Z^{m'}$ such that $\norm{B'\vec x - \vec t'}_p \leq r'$. 
    For any $r_G$, consider a vector $\vec v \in \ballp{\ldgr, (r_G^p - 1 - r'^p)^{1/p}, \tdgr}$ such that $\vec v = \dgr B \vec y$ for some $\vec y \in \Z^{d'}$. Then the vector $\vec u := B \cdot (\vec x, \vec y, 1)$ satisfies
    $$ \normpp{\vec u} \leq \normpp{B'\vec x - \vec t} + \normpp{\dgr B \vec y - \tdgr} + 1 \leq r_G^p. $$
    Therefore, $\vec u \in \ballp{\lat, r_G, \vec 0}$. Since this mapping between $\vec v$ and $\vec u$ is injective, we have that
    $$ \nump{\lat, r_G, \vec 0} \geq \nump{\dgr B, (r_G^{p} - 1 - r'^p)^{1/p}, \tdgr}. $$
    This completes the proof of item 1. 
    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
    Next, suppose that the input $\cvp_{p, \gamma'}$ instance was a \no instance. This implies that $\dist(\cL', \vec t') > \gamma' r'$. 
    For any $r_A$, let $\vec u \in \ballp{\lat, r_A, \vec 0}$ such that $\vec u = (B'\vec x, B^\dagger \vec y , \cl)$ for some $\vec x \in \Z^{m'},~\vec y\in\Z^{d'}$ and $\cl\in \Z$. We have 
    \[ \normpp{\vec u} \leq \normpp{B'\vec x - \cl\vec t'} + \normpp{\dgr B \vec y - \cl\tdgr} + \cl^p \leq r_A^p, \]
    which implies that 
    \[ \normpp{B'\vec x - \cl \vec t'} \leq r_A^p - \cl^p \leq r_A^p; \]
    \begin{equation}
    \label{eqn:coeffForGadget}
     \normpp{\dgr B \vec y - \cl \vec t^{\dagger}} ~\leq ~r_A^p - \cl^p - (\dist_p(\lat', \ell \vec t'))^p ~\leq ~r_A^p - (\dist_p(\lat', l \vec t'))^p.
     \end{equation}
    Since $\lat' \subseteq \Z^m$, and $\cl \vec t' \in \Z^m$, we have that the number of values that $B'\vec x$ can take is 
    \begin{align}
        \nump{\lat', r_A, \cl \vec t'} \notag &\leq \nump{\Z^m, r_A, \cl \vec t'} && (\because \lat' \subseteq \Z^m) \notag \\
        &= \nump{\Z^m, r_A, \vec 0} && (\because \cl\vec t' \in \Z^m) \label{eqn:svptemp1}.
    \end{align}
    
    Let $S_\cl$ be the set of points in $\lat$ of length at most $r_A$ such that their last coordinate is $\cl$. Observe that $\abs{S_\cl} = \abs{S_{-\cl}}$. 
    Then, 
    $$ \nump{\lat, r_A, \vec 0} \leq \sum_{\cl=-\floor{r_A}}^{\floor{r_A}} \abs{S_\cl} \leq 2 \sum_{\cl = 0}^{\floor{r_A}} \abs{S_\cl}. $$

    \textbf{Suppose that $\cl$ is even.} Then $\vec t' \in \lat' / 2 \implies \dist_p(\lat', \cl\vec t') = 0$. Thus, we have that the number of possible values $\vec B^\dagger y$ can take is at most,
    \begin{align}
        \label{eqn:svptemp2}
        \nump{\ldgr, r_A, \cl \tdgr}.
    \end{align}
    The number of possible vectors $\vec u$ in this case is at most the product of \cref{eqn:svptemp1} and \cref{eqn:svptemp2},
    \begin{align}
        \label{eqn:svpslodd}
        \abs{S_l} \leq \nump{\Z^m, r_A, \vec 0} \nump{\ldgr, r_A, \cl\vec {t}^\dagger}.
    \end{align}
    \textbf{Suppose that $\cl$ is odd.} Then $\vec t' \in \lat' / 2 \implies \cl\vec t' \in \lat' + \vec t'$. Let $\cl = 2z+1$. We have that
    $$\dist_p(\lat', (2z+1)\vec t') = \dist_p(\lat', \vec v' + \vec t') = \dist_p(\lat', \vec t'),$$
    where $\vec v' \in \lat'$. 
    Therefore, the number of possible values $B^\dagger \vec y$ can take while satisfying \cref{eqn:coeffForGadget} is at most 
    % \rnote{Can you elaborate more on this step}
    \begin{align}
        \label{eqn:svptemp3}
        % \nump{\ldgr, (r_A^p - \cl^p - (\gamma' r')^p)^{1/p}, \cl \tdgr} \leq 
        \nump{\ldgr, (r_A^p - (\gamma' r')^p)^{1/p}, \cl \tdgr}.
    \end{align}
    The number of possible vectors $\vec u$ in this case is at most the product of \cref{eqn:svptemp1} and \cref{eqn:svptemp3},
    \begin{align}
        \label{eqn:svpsleven}
        \abs{S_l} \leq \nump{\Z^m, r_A, \vec 0} \nump{\ldgr, (r_A^p - (\gamma' r')^p)^{1/p}, \cl\tdgr}.
    \end{align}
    Thus summing over even and odd $\cl$ from \cref{eqn:svpslodd} and \cref{eqn:svpsleven} we get an upper bound on $\nump{\lat, r_A, \vec 0}$ as,
    \begin{align*}
        &\leq  2\cdot \nump{\Z^m, r_A, \vec 0} { \sum_{j=0}^{\lceil r_A/2 \rceil}\paren{\nump{\ldgr,~(r_A^p - (\gamma' r')^p)^{1/p}, (2j+1)\cdot \tdgr} + \nump{\ldgr, r_A, (2j) \cdot \vec{t}^\dagger} }}\\
        &\leq(r_A +4) \cdot \nump{\Z^m, r_A, \vec 0} \cdot \paren{\max_{\cl_1 \in \Z}\left\{\nump{\ldgr,~(r_A^p - (\gamma' r')^p)^{1/p}, \cl_1\cdot \tdgr} \right\} + \max_{\cl_0 \in 2\Z}\left\{  \nump{\ldgr, r_A, \cl_0 \cdot \vec{t}^\dagger} \right\}}
    \end{align*}
    This completes the proof of item 2.
\end{proof}

% \dnote{We should have a corollary here saying that the number of short vectors in the YES case are exponentially more than the number of short vectors in the NO case. A lot of the calculations, particularly Claim 4.5 in the following theorem will appear in this corollary. Also, don't throw this to the appendix. }

%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%

This gives us the following lemma, that says that for any $\lin_\varepsilon$ instance, we can efficiently compute a lattice such that the number of short vectors in the \yes case are exponentially more than the number of short vectors in the \no case. 

\begin{lemma}
    \label{lem:AGRelation}
    For all $p \in (2,\infty)$ , there is an efficient algorithm that takes as an input a $\lin_\varepsilon$ instance $(M, \vec v)$ over $\F_2$ in $n$ variables and $m = \order{n}$ equations, and outputs $(B, r, \gamma, A, G)$ where $B$ generates a lattice $\lat$ in $\order{n}$ dimensions, $\gamma > 1$ is a constant, $r > 0$ is a radius, and constants $A,~G$ are such that $G \geq 2^m A$ and 
    \begin{enumerate}
        \item if it was a \yes instance of $\lin_\varepsilon$ then, $\nump{\lat, r, \vec 0} \geq G$;
        \item if it was a \no instance of $\lin_\varepsilon$ then, $\nump{\lat, \gamma r, \vec 0} \leq A$.
    \end{enumerate}
\end{lemma}

\begin{proof}
    Fix a $p$. We describe the algorithm followed by correctness. 

    \textbf{Algorithm.}
    Define $\gamma' := \paren{1 + \frac{8\varepsilon}{3}}^{1/p}$.
    On input a $\lin_\varepsilon$ instance $M \in \F_2^{m \times n},~\vec v \in \F_2^m$, the reduction computes a $\cvp_{p, \gamma'}$ instance $(B', \vec t', r')$ using the algorithm from \cref{thm:LinCvpReduction}.
    Recall from the proof of \cref{thm:LinCvpReduction} that if this instance is a \yes instance, then $\dist_p(\lat(B'), \vec t') \leq r'$, and if this instance is a \no instance then $\dist_p(\lat(B'), \vec t') \geq (\gamma' r')$. 
    Also recall that by construction in \cref{thm:LinCvpReduction}, $B' \in \Z^{m \times (n+m)}$, $r' = {(3m/8)^{1/p}}$, $2\Z^m \subseteq \lat(B') \subseteq \Z^m$ and $\vec t' \in \lat(B') / 2$ as $\vec t' \in \Z^m$.
    Therefore, this instance satisfies the conditions for \cref{lem:cvpToSvp} to hold. 
    The reduction then applies the transformation in \cref{lem:cvpToSvp} with $r_G=r$, $ r_A= \gamma r$, $B^\dagger= \alpha I_d$ and $\tdgr=\alpha t\cdot \vec{1}_d$ on this $\CVP_{p,\gamma}$ instance, for a particular choice of efficiently computable parameters $\alpha$, $t$, $r$, $\gamma$ and $d$ (to be determined in what follows), and gets a generating set $B$ of a lattice $\lat$ in $m + d + 1$ dimensions. 
    Define,
    \begin{equation}
        \label{eqn:svpGood}
    G := \nump{\ldgr, (r^{p} - 1 - r'^p)^{1/p}, \tdgr},
\end{equation}
    \begin{align}
        \label{eqn:svpAnnoying}
        A := (\gamma r+4) \cdot \nump{\Z^m, \gamma r, \vec 0} \cdot \bigg(&\max_{\cl_1 \in \Z}\left\{\nump{\ldgr,~((\gamma r)^p - (\gamma' r')^p)^{1/p}, \cl_1\cdot \tdgr} \right\} + \notag \\
        &\max_{\cl_0 \in 2\Z}\left\{  \nump{\ldgr, \gamma r, \cl_0 \cdot \vec{t}^\dagger} \right\}\bigg). 
    \end{align}
    The reduction outputs $(B, \gamma, r, A, G)$. Efficiency is clear, as $A$ and $G$ can be approximated efficiently using the theta function. We will now prove the correctness. 

    \textbf{Correctness.}
    Notice that $G$ and $A$ are simply the RHS of \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo} respectively. \Cref{eqn:svpGood} and \cref{eqn:cvpToSvpYes} imply that if the input was a \yes instance of $\lin_\varepsilon$, then $$\nump{\lat, r, \vec 0} \geq G.$$
    Similarly, \cref{eqn:svpAnnoying} and \cref{eqn:cvpToSvpNo} imply that if the input was a \no instance of $\lin_\varepsilon$, then $$\nump{\lat, \gamma r, \vec 0} \leq A.$$
    Let $\delta$ and $C_r$ be as in \cref{thm:SvpIntegerGadget_new} for the parameters $(p, \sigma=\gamma'^p)$. Fix $r, \gamma$ such that 
    $$r^p = \svprval; \quad \quad \gamma^p = \svpgammaval.$$
    By \cref{lemma:theta0}, for any $\gamma r,~\tau$, there exists a $K > 0$ which is independent of $m$, such that 

    \begin{align}
        \nump{\Z^{m}, \gamma r, \vec 0} &\leq \exp(\tau (\gamma r)^p) \Theta(\tau, \vec 0) \notag \\ 
        &= \exp(\tau (\gamma r)^p) \Theta(\tau, 0)^{m} \notag \\ 
        &\leq K^{m} && (\because r^p \in \order{m}).
    \label{eqn:numpKsvp}
    \end{align}

    Let $\phi_0, \phi_1$ and $t$, be the constants from \cref{thm:SvpIntegerGadget_new} for the particular $p$.
    Set $$d = \max\left\{ \ceil{\log_{\phi_0}(3K)}, \ceil{\log_{\phi_1}(3K)} \right\} m,$$ and let $~\dgr r = C_r \cdot(d)^{1/p}$. Note that $d = \order{m}$.
    A simple but tedious calculation shows that the following is true.
    \begin{restatable}{claim}{claimSvpGadgetParam}
        \label{claim:SvpGadgetParameter}
        For any $p,\gamma', r'$, if we set 
        \begin{align*}
        \alpha^p = \svpalphaval;
        \quad \quad r^p = \svprval; 
        \quad \quad \gamma^p = \svpgammaval;
    \end{align*}
    then the following holds. 
    \begin{enumerate}
        \item $\left(r^{p} - 1 - r'^p\right)^{1/p} \geq (1-\delta)^{1/p} (\alpha r^{\dagger})$. \label{im:svpRadii1}
        \item $\gamma r \leq \alpha r^{\dagger}$ \label{im:svpRadii2}
        \item $\left((\gamma r)^p - (\gamma' r')^p \right)^{1/p}\leq (1 - \delta\sqrt{\gamma'^p})^{1/p} (\alpha r^{\dagger})$ \label{im:svpRadii3}
    \end{enumerate}
    \end{restatable}

    To see \cref{im:svpRadii1} notice that,
    \begin{align*}
        r^p-1-r'^p&= \left(1-\frac{\delta}{2} \right)\frac{ 2r'^p}{\delta} - r'^p =2\frac{(1-\delta)}{\delta}r'^p= (1-\delta)(\alpha r^\dagger)^p.
    \end{align*}
    To see \cref{im:svpRadii2}, notice that since $r'^p=\Omega({m})$, we can assume that $(1+\delta/100)\leq r'^p/10$. This implies,
    \begin{align*}
        (\gamma r)^p &\leq \left(1+\delta/100\right)\left(1+\left(1-\frac{\delta}{2}\right)\frac{2r'^p}{\delta}\right)\\
        &\leq \frac{ r'^p}{10}+\left(1+\delta/100\right)\left(\left(1-\frac{\delta}{2}\right)\frac{2r'^p}{\delta}\right)\\
        & \leq \paren{\frac{\delta}{10}+\paren{1+\frac{\delta}{100}}\paren{2-\delta}}\left(\frac{r'^p}{\delta}\right)\\
        &=\paren{2-\frac{22}{25}\delta-\frac{\delta^2}{100}}\paren{\frac{r'^p}{\delta}}\\
        &< \paren{\frac{2r'^p}{\delta}}\\
        &= (\alpha r^\dagger)^{p}.
    \end{align*}
    For \cref{im:svpRadii3}, use the fact $\gamma^p \leq 1+\delta\cdot \frac{(\sqrt{\gamma'}-1)^2}{2}$ and $\gamma'\geq 1$. Again, since $r'^p=\Omega({m})$ , without loss of generality we can assume that, $\frac{\delta\paren{\sqrt{\gamma'^p}-1}^2 r'^p}{2}\geq \gamma^p$. Hence we get,
    \begin{align*}
        (\gamma r)^p &\leq \paren{\frac{2r'^p}{\delta}}\paren{\paren{1-\frac{\delta}{2}}\paren{1+\delta\cdot \frac{(\sqrt{\gamma'^p}-1)^2}{2}}}+\gamma^p\\
        &= \paren{\frac{2r'^p}{\delta}} \paren{\paren{1-\delta\sqrt{\gamma'^p}}+\paren{\frac{\delta \gamma'^p}{2}+\frac{\delta^2 \sqrt{\gamma'^p
        }}{2}}-\paren{\frac{\delta(\delta+\delta \gamma'^p)}{4}}}+\gamma^p\\
        &= \paren{\frac{2r'^p}{\delta}} \paren{\paren{1-\delta\sqrt{\gamma'^p}} + \frac{\delta \gamma'^p}{2} -\frac{\delta^2\paren{\sqrt{\gamma'^p}-1}^2}{4}}+\gamma^p\\
        &=(1 - \delta\sqrt{\gamma'^p}) (\alpha r^{\dagger})^p+(\gamma'r')^p- \frac{\delta\paren{\sqrt{\gamma'^p}-1}^2 r'^p}{2}+\gamma^p\\
        &\leq (1 - \delta\sqrt{\gamma'^p}) (\alpha r^{\dagger})^p+(\gamma'r')^p .
    \end{align*}
This concludes the proof of the claim.
\Cref{im:svpRadii1} implies that 
        \begin{align}
        \label{eqn:GZBound}
        G = \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, {\alpha}{t}\cdot \vec{1}_{d}} \geq \nump{\alpha \Z^{d}, (1-\delta)^{1/p}\alpha r^{\dagger}, {\alpha}{t} \cdot\vec{1}_{d}}.
        \end{align}
        %%%%%%%%%%%%%%
        \Cref{im:svpRadii2,im:svpRadii3} and \cref{eqn:numpKsvp} imply that
        \begin{align*}
        \label{eqn:AZbound}
            A &= (\gamma r+4) \cdot \nump{\Z^m, \gamma r, \vec 0} \cdot \bigg(\max_{\cl_1 \in \Z}\left\{\nump{\ldgr,~((\gamma r)^p - (\gamma' r')^p)^{1/p}, \cl_1\cdot \tdgr} \right\} +  \max_{\cl_0 \in 2\Z}\left\{  \nump{\ldgr, \gamma r, \cl_0 \cdot \vec{t}^\dagger} \right\}\bigg) \notag \\
            &\leq  (\gamma r+4) K^m  \bigg( \max_{\cl_1 \in \Z} \left\{\nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, {\alpha}{\cl_1 t} \cdot \vec{1}_{d}}\right\}+ \max_{\cl_0 \in 2\Z} \left\{ \nump{\alpha \Z^{d}, \alpha r^{\dagger}, {\alpha}{\cl_0 t} \cdot \vec{1}_{d}} \right\}\bigg) \\
            &\leq  (\gamma r+4)K^m \paren{\dfrac{1}{\phi_1^{d}} + \dfrac{1}{\phi_0^{d}}}\nump{\alpha \Z^{d}, (1-\delta)^{1/p}\alpha r^{\dagger}, {\alpha}{t} \cdot\vec{1}_{d}}\\
            &\leq (\gamma r +4)\paren{\frac{2}{3^m}}\cdot G
        \end{align*}
        For our choice of $d, \dgr r, \delta$, together with \cref{eqn:SvpIntegerGadgetCond_new}, and the fact that $r = \order{m^{1/p}}$, these imply that for a sufficiently large $m$, $G \geq 2^m A$.
\end{proof}


%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%


\begin{theorem}
    \label{thm:linToSvp}
    For any $p > 2$, there exists a constant $\gamma > 1$ such that for all $n \in \Z^+$, there is a polynomial time randomized Karp reduction from $\lin_\varepsilon$ in $n$ variables and $\order{n}$ equations to $\svp_{p, \gamma}$ in a lattice of rank $\order{n}$.
\end{theorem}

% \adi{Perhaps change $\dgr m$ to $d$ everywhere in the proof.}
\begin{proof} Fix a $p$. We first describe the algorithm, and then show correctness. 

    \textbf{Algorithm.}
%     Fix a $p$, define $\gamma' := \paren{1 + \frac{8\varepsilon}{3}}^{1/p}$.
%     On input a $\lin_\varepsilon$ instance $M \in \F_2^{m \times n},~\vec v \in \F_2^m$, the reduction computes a $\cvp_{p, \gamma'}$ instance $(B', \vec t', r')$ using the algorithm from \cref{thm:LinCvpReduction}.
%     Recall from the proof of \cref{thm:LinCvpReduction} that if this instance is a \yes instance, then $\dist_p(\lat(B'), \vec t') \leq r'$, and if this instance is a no instance then $\dist_p(\lat(B'), \vec t') \geq (\gamma' r')$. 
%     Also recall that by construction, $\rank(\lat(B')) = m$, $\lat(B') \subseteq \Z^m$, $\vec t' \in \lat(B') / 2$ and $\vec t' \in \Z^m$.
%     We claim that by applying the transformation from \cref{lem:cvpToSvp} for a particular choice of efficiently computable parameters $\alpha$, $r$, $\gamma$ and $d$ (to be determined in what follows), the reduction can find a lattice $\lat$ of rank $\order{n}$ that satisfies the conditions in equations \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo}. 
%     Define
%     \begin{equation}
%         \label{eqn:svpGood}
%     G := \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}},
% \end{equation}
%     \begin{align}
%         \label{eqn:svpAnnoying}
%         A &:= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \\ 
%         &\geq \paren{\floor{\gamma r} + 1} \nump{\Z^m, \gamma r, \vec 0} \paren{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}} + \nump{\alpha \Z^{d}, \gamma r, \vec 0} }. \notag
%     \end{align}
%     Notice that $G$ and $A$ are simply the RHS of \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo} respectively. \Cref{eqn:svpGood} and \cref{eqn:cvpToSvpYes} imply that if the input was a \yes instance of $\lin_\varepsilon$, then $$\nump{\lat, r, \vec 0} \geq G.$$
%     Similarly, \cref{eqn:svpAnnoying} and \cref{eqn:cvpToSvpNo} imply that if the input was a \no instance of $\lin_\varepsilon$, then $$\nump{\lat, \gamma r, \vec 0} \leq A.$$
The reduction uses the algorithm from \cref{lem:AGRelation} to compute $(B, \gamma, r, A, G)$. Then it
    % The reduction computes such a lattice, and then 
    samples a prime number $$q \in [\sqrt{AG} / 42,~42\sqrt{AG}],$$
    and uses the algorithm from \cref{lem:svpSparcification2} to get a basis $B'$ of sparse sub-lattice lattice $\lat' \subseteq \lat$ of rank $\order{n}$, and outputs $(B', r)$. The efficiency follows from the efficiency of \cref{lem:AGRelation} and \cref{lem:svpSparcification2}. We now prove correctness. 
    % The three transformations used by the reduction (\cref{thm:LinCvpReduction}, \cref{lem:cvpToSvp} and \cref{lem:svpSparcification2}) are efficient in $n$, therefore reduction is efficient. We now show correctness, and help her choose $\alpha$, $r$, $\gamma$ and $d$.
    % so that the number of ``good" vectors in the \yes case is much larger than the number of ``annoying" vectors in the \no case. 
    % Then the lattice $\lat$ can be sparcified using randomized process from \cref{lem:svpSparcification} to obtain another lattice $\lat''$ of rank $n''$ such that if the input $\lin$ instance was a \yes instance, with high probability at least one good vector of length at least most $r$ survives the sparcification process, and if the input $\lin$ instance was a \no instance, then with high probability all the vectors of length at most $\gamma r$ get killed.
    % In what follows, we first derive the parameters $\alpha$, $r$, $\gamma$ and $\dgr m$. We then continue to describe the action of the oracle following this transformation. 
    % We wish to lower bound the number of good vectors in the \yes case (LHS of \cref{eqn:cvpToSvpYes}) by the LSH of \cref{eqn:SvpIntegerGadgetCond}, 
    % and upper bound the number of annoying vectors in the \no case (LHS of \cref{eqn:cvpToSvpNo}) by the RHS of \cref{eqn:SvpIntegerGadgetCond}.

    % \textbf{Correctness.} 
    % Let $\delta$ be as in \cref{thm:SvpIntegerGadget} for the parameters $(p, \sigma=\gamma'^p)$. Fix $r, \gamma$ such that 
    % $$r^p = \svprval; \quad \quad \gamma^p = \svpgammaval.$$
    % By \cref{lemma:theta0}, for any $\gamma r,~\tau$, there exists a $K > 0$ such that 

    % \begin{align}
    %     \nump{\Z^{m}, \gamma r, \vec 0} &\leq \exp(\tau (\gamma r)^p) \Theta(\tau, \vec 0) \notag \\ 
    %     &= \exp(\tau (\gamma r)^p) \Theta(\tau, 0)^{m} \notag \\ 
    %     &\leq K^{m} && (\because r^p \in \order{m}).
    % \label{eqn:numpKsvp}
    % \end{align}

    % Let $\phi_0, \phi_1$ be the constants from \cref{thm:SvpIntegerGadget} for the particular $p$.
    % Set $$d = \max\left\{ \ceil{\log_{\phi_0}(3K)}, \ceil{\log_{\phi_1}(3K)} \right\} m,$$ and let $\delta,~\dgr r$ be the corresponding constants from that satisfy \cref{eqn:SvpIntegerGadgetCond}.
    % A simple but tedious calculation shows that the following is true. We defer the proof to the appendix. 
    % \begin{restatable}{claim}{claimSvpGadgetParam}
    %     \label{claim:SvpGadgetParameter}
    %     \adi{For any $p,\gamma'$?} If we set 
    %     \begin{align*}
    %     \alpha^p = \svpalphaval;
    %     \quad \quad r^p = \svprval; 
    %     \quad \quad \gamma^p = \svpgammaval;
    % \end{align*}
    % then the following holds. 
    % \begin{enumerate}
    %     \item $\left(r^{p} - 1 - r'^p\right)^{1/p} \geq (1-\delta)^{1/p} (\alpha r^{\dagger})$. \label{im:svpRadii1}
    %     \item $\gamma r \leq \alpha r^{\dagger}$ \label{im:svpRadii2}
    %     \item $\left((\gamma r)^p - (\gamma' r')^p \right)^{1/p}\leq (1 - \delta\sqrt{\gamma'^p})^{1/p} (\alpha r^{\dagger})$ \label{im:svpRadii3}
    % \end{enumerate}
    % \end{restatable}
    
    % \Cref{im:svpRadii1} implies that 
    %     \begin{align}
    %     \label{eqn:GZBound}
    %     G = \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}} \geq \nump{\alpha \Z^{d}, (1-\delta)^{1/p}\alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}.
    %     \end{align}
    %     %%%%%%%%%%%%%%
    %     \Cref{im:svpRadii2,im:svpRadii3} and \cref{eqn:numpKsvp} imply that
    %     \begin{align*}
    %     \label{eqn:AZbound}
    %         A &= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{\alpha}{2}\vec{1}_m}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \notag \\
    %         &\leq 2 (\gamma r+1) K^m \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\} \\
    %         &\leq \frac{1}{3^m} 2 (\gamma r+1) \min\{\phi_0,\phi_1\}^{d} \max \bigg\{ \nump{\alpha \Z^{d}, (1 - \delta\sqrt{\gamma'^p})^{1/p} \alpha r^{\dagger}, \frac{\alpha}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \alpha r^{\dagger}, \vec 0} \bigg\}.
    %     \end{align*}
    %     For our choice of $d, \dgr r, \delta$, together with \cref{eqn:SvpIntegerGadgetCond}, and the fact that $r = \order{m^{1/p}}$, these imply that for a sufficiently large $m$, $G \geq 2^m A$.
    \textbf{Correctness.} 
        We bound the probability of a lattice vector of a particular length making it into the sparse sub-lattice $\lat'$ lattice. 
        Suppose that the input was a $\yes$ instance of $\lin_\varepsilon$. Let $\mathcal{S}$ be the set of lattice vectors in $\lat$ of length at most $r$. 
        % These are distinct vectors of the form $\vec v_1 \oplus \vec v_2 \oplus 1$, where $\vec v_1 \in \lat(B') - \vec t' ,~\vec v_2 \in \alpha \Z^{d} - \frac{\alpha}{2}\vec 1_{d}$, and therefore they are linearly independent. Then 
        These are distinct lattice vectors such that their last coordinates are all $1$, and  $r < q \lambda_1^{(p)}(\lat)/2$ also holds\footnote{this is because $q$ grows exponentially in $m$, where as $r$ is $\order{m^{1/p}}$ }. Consider any two vectors $\vec v_1$ and $\vec v_2$ in $\mathcal{S}$. We claim that $B^{-1}(\vec v_1-\vec v_2) \neq 0 \mod q$. To see this, observe that if $B^{-1}(\vec v_1-\vec v_2) = 0 \mod q$, then $(\vec{v}_1-\vec v_2) \in q \cdot \cL(B) \implies \|(\vec{v}_1-\vec v_2)\|_p\geq q\lambda_1^{(p)}(\cL)$, which gives a contradiction by triangle inequality. This implies that the coefficient vectors of the lattice vectors in $\mathcal{S}$ are distinct and hence pairwise linearly independent in $\F_q$ because the last coordinate of coefficient vectors is also fixed to be 1. Then,
        $$\abs{\mathcal{S}} \geq G \implies \frac{q}{\abs{\mathcal{S}}} \leq {42} \cdot \sqrt{\frac{A}{G}} \in \order{-2^{m/2}}.$$
        Therefore by the lower bound in \cref{lem:svpSparcification2}, $(B', r)$ is a \yes instance of $\svp_{p, \gamma}$ except with an exponentially small probability. Next, suppose that the input was a \no instance of $\lin_\varepsilon$. Let $\mathcal{S}$ be the set of vectors of length {\em at most} $\gamma r$. We have that $\abs{\mathcal{S}} \leq A$, and hence the number of linearly independent vectors in $\mathcal{S}$ of length at most $\gamma r$ is at most $A$.
        Additionally, we claim that in this case $\gamma r \leq q \lambda_1^{(p)}(\lat)$. Too see this, suppose $\gamma r > q \lambda_1^{(p)}(\lat)$ for contradiction. This implies that $\lambda_1^{(p)}(\lat) < \frac{\gamma r}{q} < \frac{\gamma r}{A}$, because $q > A$. Let $\vec v \in \lat$ be such that $\norm{\vec v}_p = \lambda_1^{(p)}(\lat)$. Then, $\{ -A \vec v, \ldots A\vec v \}$ are $2A$ vectors of length at most $\gamma r$, contradicting the fact that $\nump{\lat, \gamma r, \vec 0} \leq A$.  
        Therefore, 
        $$ \frac{\abs{\mathcal{S}}}{q} \leq 42 \cdot \sqrt{\frac{A}{G}} \in \order{2^{-m/2}},$$
        and by the upper bound in \cref{lem:svpSparcification2}, $(B', r)$ is a \no instance of $\svp_{p, \gamma}$ except with an exponentially small probability. \qedhere

    % Together with \cref{eqn:numpthetasvp}, \cref{eqn:SvpIntegerGadgetCond} and the fact that $\gamma r = \order{r'} = \order{n}$ imply that for a sufficiently large $n$, $G \geq 2^{n'}A$. 

    % We now continue with the action of the reduction algorithm. 
    % Define $P := 10\sqrt{AG}$. The reduction does the following $\ell := \ceil{100n'\log P}$ times. It samples a prime number $q$ in the range $[10 P \log P,~20 P \log P]$, and uses the algorithm from \cref{lem:svpSparcification2} to obtain (a basis of) a sub-lattice $\lat''$ of rank $n' + d + 1 = \order{n}$.
    % Then it uses its $\svp_{p, \gamma}$ oracle to check if $\lambda_1^{(p)}(\lat'') \leq r$. It outputs \yes iff the oracle returns \yes more than $\delta \ell$ times, where
    % \[ \delta := \frac{P}{20q} - \frac{P^2}{200q^2} \geq \frac{1}{100 \log P}. \]

    % Suppose that the input $\lin_\varepsilon$ instance was a \yes instance. Then, $\lat'$ has at least $G$ vectors of length at most $r$. By the construction in \cref{eqn:cvpToSvpBasis}, these are vectors with their last coordinates as $1$, and thus are all primitive vectors. By \cref{lem:svpSparcification2}, 
    % \begin{align*}
    %     \Pr \left[ \lambda_1^{(p)}(\lat'') \leq r \right] &\geq 2 \delta.
    % \end{align*}
    % Therefore, the reduction outputs \yes except with probability at most $\exp\paren{-\Omega(d)}$ by Chernoff-Hoeffding bound. 

    % Next suppose that the input $\lin_\varepsilon$ instance was a \no instance. Then, $\lat'$ has at most $A$ vectors of length at most $\gamma r$, and thus at most $A$ {\em primitive} vectors of that length. Again by \cref{lem:svpSparcification},
    % \begin{align*}
    %     \Pr \left[ \lambda_1^{(p)}(\lat'') \leq r \right] &\leq \frac{A}{q} \leq \frac{\delta}{2}.
    % \end{align*}
    % Therefore, the reduction outputs \no except with probability at most $\exp\paren{-\Omega(d)}$, again by Chernoff-Hoeffding bound.

\end{proof}

Together with \cref{cor:linEthHard}, we get the following theorem.

\thmsvpethhard*




==> temp.tex <==
\begin{corollary}
    \label{lem:AGRelation}
    Suppose $(\cL', \vec t', r')$ is a $\cvp_{p, \gamma'}$ instance over an integer lattice of rank $n$, such that $\vec t' \in \lat' / 2$ and $\vec t' \in \Z^n$. 
    Then there exists an efficiently computable lattice $\lat$ of $\rank(\cL) = \order{n}$, and $d \in \Z^+$, constants $\gamma, \alpha > 0$ and any radius $r$, there exist efficiently computable functions $A(n),~G(n)$ such that $G(n) \geq 2^n A(n)$ and 
    \begin{enumerate}
        \item if it was a \yes instance of $\cvp_{p, \gamma'}$ then, $\nump{\lat, r, \vec 0} \geq G(n)$;
        \item if it was a \no instance of $\cvp_{p, \gamma'}$ then, $\nump{\lat, \gamma r, \vec 0} \leq A(n)$.
    \end{enumerate}
\end{corollary}

\begin{proof}
    The result follows immediately by applying the transformation from \cref{lem:cvpToSvp}. Specifically, for a particular choice of efficiently computable parameters $\alpha$, $r$, $\gamma$ and $d$ to be determined in what follows, the reduction can find a lattice $\lat$ of rank $\order{n}$ that satisfies the conditions in equations \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo}. 
    Set
    \begin{equation}
        \label{eqn:svpGood}
    G(n) = \nump{\alpha \Z^{d}, (r^{p} - 1 - r'^p)^{1/p}, \frac{\alpha}{2}\vec{1}_{d}},
\end{equation}
    \begin{align}
        \label{eqn:svpAnnoying}
        A &= 2 \paren{\gamma r + 1} \nump{\Z^m, \gamma r, \vec 0} \max \bigg\{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}}, \nump{\alpha \Z^{d}, \gamma r, \vec 0} \bigg\} \\ 
        &\geq \paren{\floor{\gamma r} + 1} \nump{\Z^m, \gamma r, \vec 0} \paren{ \nump{\alpha \Z^{d}, ((\gamma r)^p - (\gamma' r')^p)^{1/p}, \frac{1}{2}\vec{1}_{d}} + \nump{\alpha \Z^{d}, \gamma r, \vec 0} }. \notag
    \end{align}
    Notice that $G$ and $A$ are simply the RHS of \cref{eqn:cvpToSvpYes} and \cref{eqn:cvpToSvpNo} respectively. 
    \Cref{eqn:svpGood} and \cref{eqn:cvpToSvpYes} imply that if the input was a \yes instance of $\lin_\varepsilon$, then $$\nump{\lat, r, \vec 0} \geq G.$$
    Similarly, \cref{eqn:svpAnnoying} and \cref{eqn:cvpToSvpNo} imply that if the input was a \no instance of $\lin_\varepsilon$, then $$\nump{\lat, \gamma r, \vec 0} \leq A.$$
\end{proof}









We prove new hardness results for fundamental lattice problems under the Exponential Time Hypothesis (ETH). Building on a recent breakthrough by Bitansky et al. [BHIRW24], who gave a polynomial-time reduction from $\mathsf{3SAT}$ to the (gap) $\mathsf{MAXLIN}$ problem-a class of CSPs with linear equations over finite fields-we derive ETH-hardness for several lattice problems. 

First, we show that for any $p \in [1, \infty)$, there exists an explicit constant $\gamma > 1$ such that $\mathsf{CVP}_{p,\gamma}$ (the $\ell_p$-norm approximate Closest Vector Problem) does not admit a $2^{o(n)}$-time algorithm unless ETH is false. Our reduction is deterministic and proceeds via a direct reduction from (gap) $\mathsf{MAXLIN}$ to $\mathsf{CVP}_{p,\gamma}$.

Next, we prove a randomized ETH-hardness result for $\mathsf{SVP}_{p,\gamma}$ (the $\ell_p$-norm approximate Shortest Vector Problem) for all $p > 2$. This result relies on a novel property of the integer lattice $\mathbb{Z}^n$ in the $\ell_p$ norm and a randomized reduction from $\mathsf{CVP}_{p,\gamma}$ to $\mathsf{SVP}_{p,\gamma'}$.


Finally, we improve over prior reductions from $\mathsf{3SAT}$ to $\mathsf{BDD}_{p, \alpha}$ (the Bounded Distance Decoding problem), yielding better ETH-hardness results for $\mathsf{BDD}_{p, \alpha}$ for any $p \in [1, \infty)$ and $\alpha > \alpha_p^{\ddagger}$, where $\alpha_p^{\ddagger}$ is an explicit threshold depending on $p$. 

We additionally observe that prior work implies ETH hardness for the gap minimum distance problem ($\gamma$-$\mathsf{MDP}$) in codes. 





We prove new hardness results for fundamental lattice problems under the Exponential Time Hypothesis (ETH). Building on a recent breakthrough by Bitansky et al. [BHIRW24], who gave a polynomial-time reduction from 3SAT to the (gap) MAXLIN problem—a class of CSPs with linear equations over finite fields—we derive ETH-hardness for several lattice problems.

First, we show that for any $p \in [1, \infty)$, there exists an explicit constant $\gamma > 1$ such that CVP$_{p,\gamma}$ (the $\ell_p$-norm approximate Closest Vector Problem) does not admit a $2^{o(n)}$-time algorithm unless ETH is false. Our reduction is deterministic and proceeds via a direct reduction from (gap) MAXLIN to CVP$_{p,\gamma}$.

Next, we prove a randomized ETH-hardness result for SVP$_{p,\gamma}$ (the $\ell_p$-norm approximate Shortest Vector Problem) for all $p > 2$. This result relies on a novel property of the integer lattice $\mathbb{Z}^n$ in the $\ell_p$ norm and a randomized reduction from CVP$_{p,\gamma}$ to SVP$_{p,\gamma'}$.

Finally, we improve over prior reductions from 3SAT to BDD$_{p, \alpha}$ (the Bounded Distance Decoding problem), yielding better ETH-hardness results for BDD$_{p, \alpha}$ for any $p \in [1, \infty)$ and $\alpha > \alpha_p^{\dagger\dagger}$, where $\alpha_p^{\dagger\dagger}$ is an explicit threshold depending on $p$.

We additionally observe that prior work implies ETH hardness for the gap minimum distance problem ($\gamma$-MDP) in codes.




We prove new hardness results for fundamental lattice problems under the Exponential Time Hypothesis (ETH). Building on a recent breakthrough by Bitansky et al. (BHIRW24), who gave a polynomial-time reduction from 3SAT to the (gap) MAXLIN problem—a class of CSPs with linear equations over finite fields—we derive ETH-hardness for several lattice problems.

First, we show that for any $p \in [1, \infty)$, there exists an explicit constant $\gamma > 1$ such that CVP$T_{p,\gamma}$ (the $\ell_p$-norm approximate Closest Vector Problem) does not admit a $2^{o(n)}$-time algorithm unless ETH is false. Our reduction is deterministic and proceeds via a direct reduction from (gap) MAXLIN to CVP$T_{p,\gamma}$.

Next, we prove a randomized ETH-hardness result for SVP$T_{p,\gamma}$ (the $\ell_p$-norm approximate Shortest Vector Problem) for all $p > 2$. This result relies on a novel property of the integer lattice $\mathbb{Z}^n$ in the $\ell_p$ norm and a randomized reduction from CVP$T_{p,\gamma}$ to SVP$T_{p,\gamma'}$.

Finally, we improve over prior reductions from 3SAT to BDD$T_{p, \alpha}$ (the Bounded Distance Decoding problem), yielding better ETH-hardness results for BDD$T_{p, \alpha}$ for any $p \in [1, \infty)$ and $\alpha > \alpha_p^{\dagger\dagger}$, where $\alpha_p^{\dagger\dagger}$ is an explicit threshold depending on $p$.

We additionally observe that prior work implies ETH hardness for the gap minimum distance problem ($\gamma$-MDP) in codes.
